LLM Routing with Dueling Feedback

We study LLM routing, the problem of selecting the best model for each query while balancing user satisfaction, model expertise, and inference cost. We formulate routing as contextual dueling bandits, learning from pairwise preference feedback rather than absolute scores, thereby yielding label-efficient and dynamic adaptation. Building on this formulation, we introduce Category-Calibrated Fine-Tuning (CCFT), a representation-learning method that derives model embeddings from offline data using contrastive fine-tuning with categorical weighting. These embeddings enable the practical instantiation of Feel-Good Thompson Sampling for Contextual Dueling Bandits (FGTS.CDB), a theoretically grounded posterior-sampling algorithm. We propose four variants of the categorical weighting that explicitly integrate model quality and cost, and we empirically evaluate the proposed methods on the RouterBench and MixInstruct datasets. Across both benchmarks, our methods achieve lower cumulative regret and faster convergence, with better robustness and performance-cost balance than strong baselines built with a general-purpose OpenAI embedding model.

==> iclr2026/01_introduction_0910.tex <==
\section{Introduction Old--1}
\label{sec:intro_old1}

\textsc{\rcmt{The Importance of Routing and the Double Response Setting}}

\rcmt{(The importance of routing)}
The potential of LLMs is so large that it almost becomes a necessary part of daily life.
As online users, we ask them all sorts of questions to obtain the information we need.
As a service provider, we want to generate satisfying replies with minimum cost.
Before the emergence of a universally dominant and affordable foundation model\footnote{[TI] Even if a universally dominant and affordable and zero latency foundation model may be available in the future, such models may internally have routing mechanisms. OpenAI decided to add a router to different models within the GPT-5 system, so it's 1 natural future path. This means our research may help the society to reach the universally dominant model in the future. Maybe we can say something like this whenever someone attacks us with the argument of a universally dominant model. \url{https://cdn.openai.com/gpt-5-system-card.pdf}}, routing is an important problem as different LLMs have respective expertise (strengthnesses) \bcmt{(cite routerbench and mix-instruct)} and different cost (weaknesses) \bcmt{(cite routerbench)}.
Studying how to weigh these factors and choose the best candidate is the core of the routing problem.

\rcmt{(Viewing the users' and the service providers' goals as a whole)}
The LLM routing problem is essentially a matching problem.
The matching optimizes toward two fronts.
On the user side, we need to consider different users' preferences.
On the service provider's side, we need to consider the agent's capability and the employment cost. 
The three factors (the user's preference, the agent's expertise, and the agent's cost) combined to form a complex and, most of the time, unknown utility function.
Since we don't know the utility function, let alone optimizing it to solve the matching problem.

\rcmt{(Relevant papers -- Part 1: supervised learning, online learning, double response. Will be later (i.e., Part 2) contrasted with the CDB setting)}
At the beginning, a machine learning approach was proposed in the single response scenario as long as one has a good estimate for the utility function \bcmt{(various ways such as modeling, pseudo-labeling, etc to estimate the utility)}.
An online learning approach was taken to learn the utility function and the LLM selection strategy on the fly.

Sometimes, even the user does not know the utility function.
For instance, when a question is open-ended.
In such a case, the double response scenario was proposed to collect supervision for learning.
\rcmt{In fact, practically, an LLM more often asks for pairwise preference feedback than a rating scale feedback (this is the main reason we choose double response).}
The advantage of adopting double response is that only one click is required instead of providing a hard-to-calculate real value.
Moreover, it is more confident to say reply A is better than B than to say reply A is in third place out of the scores of ten.
Despite being practically appealing, we noticed that not much investigation has been done for this setting. 

\begin{itemize}
    \item Single response scenario + supervised learning approach(es): routing methods
    \item Double response scenario + supervised learning approach(es): importance of the double response setting
    \item Single response scenario + Online learning(es): importance of the online approach
    \item Double response scenario + Online learning approach(es): This paper's MAIN topic
    \item \bcmt{Do we discuss different benchmarks?}
\end{itemize}

\rcmt{(Mention literature papers; the first 3 bullets above; more on stating differences rather than in-depth comparisons)}
Papers take real-valued scores and train via supervised learning (the beginner papers).
Papers study preference feedback (what are their cons?).
\bcmt{(Save this 3rd one later)} Papers using online learning but only consider a very primitive setting where two arms are considered (also not on real-world benchmarks?).

\subsection{Background}

\textsc{\rcmt{The Importance of the CDB Approach}}

\bcmt{(What motivates our problem setting.)}
\bcmt{(Start with the data nature. Then, argue the importance of our setting (not only the online learning alone, but also the dueling feedback and contextual information). Can I find 3 good reasons?)}
(1) Small labeling cost (only needs binary feedback).
(2) Contextual structure (semantic information) in the question sequence. 
One should choose an LLM whose expertise matches the characteristics of the question.
(3) The changing nature and the size of online users.
(4) A fixed model would suffer from distribution shift, while an online learner can adapt the environment on the fly.

\rcmt{(Our setting. Problem formulation and assumptions.)}
We choose the contextual dueling bandit to capture the nature of the routing problem mentioned above.

\rcmt{(For CDB, we adapt a latest method called FGTS.CDB. A brief introduction.)}
What is contextual bandit?
What is a dueling bandit?
What is FGTS and what is FGTS.CDB?
\bcmt{(cite [T. Zhang] and [FGTS.CDB] papers.)}
FGTS was first proposed by [T. Zhang] with a distinctive ``feel-good'' term that up-weights the model with good performance history.
[FGTS.CDB] extended FGTS to the dueling setting, hence the ``CDB'' in the proposed algorithm's name.
Both papers focused on the theory of FGTS.
An important scientific perspective for investigating this problem is to understand how to translate binary feedback into an LLM selection strategy as if the utility function is given.

\rcmt{(Send the algorithm to background?)}
\begin{algorithm}
\caption{FGTS.CDB}\label{alg:fgts-cdb}
\begin{algorithmic}[1]
\State Given hyperparameters $\eta, \mu$. Initialize $S_0 = \varnothing$.
\For{$t = 1, \ldots, T$}
  \State Receive prompt $x_t$ and action space $\mathcal{A}_t$.
  \For{$j = 1, 2$}
    \State Sample model parameter $\theta_t^{j}$ from the posterior distribution $p^{j}(\,\cdot \mid S_{t-1})$, defined in (4.1).
    \State Select response $a_t^{j} = \arg\max_{a \in \mathcal{A}_t}\; \langle \theta_t^{j}, \,\phi(x_t,a) \rangle$.
  \EndFor
  \State Receive preference $y_t$.
  \State Update dataset $S_t \leftarrow S_{t-1} \cup \{(x_t, a_t^{1}, a_t^{2}, y_t)\}$.
\EndFor
\end{algorithmic}
\end{algorithm}

\subsection{Paper Contributions}

\rcmt{(Realistic challenges)}
Recall that the success hinges on translating the information in binary feedback to the regret-defining utility function.
Theoretically speaking, the connection is specified by Assumption-? in [FGTS.CDB].
The intuition is that, when a correct feature function $\phi$ is given, the correct parameter $\theta^*$ can be learned in an online fashion.
This assumption leads to the regret bounds Theorem-? and Theorem-? proved by [FGTS.CDB].

\rcmt{(To address the challenge, our proposition and its coverage is as follows. A summary of our contributions.)}
On the practical side, it is not clear how to build the question embedding $x_t$, the model embedding $a$, and the feature function $\phi$.
\bcmt{(Contribution 1)} In this paper, we propose a generic method to construct the feature function, which is covered by Section~\ref{sec:generic_method}.
\bcmt{(Contribution 2)} The feature function facilitates the construction of the first trainable contextual dueling learner in LLM routing.
\bcmt{(Contribution 3)} The effectiveness of the proposed method is verified by two real-world datasets, which will be elaborated in Section~\ref{sec:experiments}
\bcmt{(Contribution 4)} The proposed method is tested via common practices, including prompting, context fine-tuning, open-sourced and closed-sourced text embeddings, accumulating substantial knowledge of addressing LLM routing.



\subsection{Outline}
\begin{itemize}
    \item Storyline (Introduction)
    \item Background
    \item Terminologies, notation, symbols
\end{itemize}

\subsection{Key Arguments}
Version 2
\begin{itemize}
    \item The importance of LLM routing
    \item The importance of CDB setting
    \begin{itemize}
        \item (C: represent user satisfactory, model expertise) How to encode the question's semantic information? How others ``contextualize'' the information they want?
        \item (D: different feedback) Compare two settings: train with user feedback scores vs train with preference feedback. We need a moderate-sized offline dataset with scores and a large online testing dataset with preference feedback.
        \item (B: online vs offline) Online adaptation and robust generalization (for distribution shift).
        \item (model embedding design) Multi-objective Optimization: Considering performance + $\lambda$ cost vs only performance
    \end{itemize}
    \item We can (1) robust generalization, and (2) accommodate new LLM (by calling a public benchmark).
    \item Minor comparisons (1) 2 arms vs K arms (bandits). (2) preference feedback of strong/weak vs preference of K LLMs (pairwise feedback).
    \item Grounding a theoretical justified approach with constructive strategy
    \item Obtain efficacy evidence from real-world datasets.
\end{itemize}

Version 1
\begin{itemize}
    \item The importance of the routing problem
    \item The advantage of online approach over SL approach \rcmt{(What is it?)}
    \item The extension from 2 arms to K arms
    \item The verification on 2 real-world datasets (vs simulations with artificial data)
    \item A generic and practical feature construction strategy (vs theory guarantees)
\end{itemize}







==> iclr2026/02_intro.tex <==


\section{Introduction}
\label{sec:intro}
The potential of LLMs is so large that it almost becomes a necessary part of daily life, with applications from office assistance, fashion/dining suggestions, to entertainment.
LLM routing refers to a problem of dynamically selecting the most suitable LLM from a set of candidates for each query from a sequence of questions.
Before the emergence of a universally dominant and affordable foundation model, routing is important as a suitable LLM matches the user traits, the model expertise, and the cost.
To balance these three key factors, cascading algorithms \cite{FrugalGPT} and \cite{AutoMix} were first proposed.
The idea is to query a cheap model first and advance the query to a more expensive model if the current reply is likely to fail the user’s expectation.

A drawback of cascading is the accumulated cost and latency caused by a series of calls to multiple LLM candidates to obtain the final reply to output.
To avoid this, supervised routing methods \cite{2309.15789, zooter, hybridLLM, RouterBench, 2405.00467} were proposed.
In general, a supervised router reduces the latency by applying a classification or a regression prediction before the LLM query.
The supervised approach has evolved into branches. 
A branch studied ensembles \cite{LLM-Blender, SelectLLM, Avengers}, which allows the agent to select a subset or fuse answers. 
Another branch exercised cost-aware model assignment \cite{FORC, RouterBench, OptLLM} to balance the cost and performance.
There are also works that combine representation learning \cite{GraphRouter, EmbedLLM} to strengthen the user and model’s semantic information before training.

For supervised routing methods, having abundant real-valued annotations with high-quality label information is critical for successful classification or regression training.
Unfortunately, such a requirement is often unrealistic in the context of LLM routing.
In some cases, users are either reluctant or unmotivated to provide feedback. 
They may also be unable to quantify their satisfaction, especially when dealing with open-ended questions or when they lack the ability to verify the correctness of the LLM's response.
To ease the annotation burden, some efforts focused on weak supervision \cite{RouteLLM, Eagle, MixLLM}, which only collect binary feedback such as like/dislike or pairwise comparison.
The advantage is that one-click feedback is user-friendly, and it is more confident to say reply A is better than B than to assign reply A a score out of ten.
The reason that makes a weakly supervised approach appealing is that, as shown by the referred papers, the binary feedback can be translated into a model ranking or an estimate of the labeling function. 

In addition to the challenge of annotation, adaptivity remains a key challenge to be addressed in developing a usable routing system.
Shifts in query distributions, such as changes in trending topics like fashion or temporal variations between work hours and leisure time, introduce non-stationary conditions. 
Moreover, new LLMs and benchmarks are continuously introduced, resulting in a constantly evolving environment for routing.
These evolving conditions often exceed the capacity of static, supervised learning-based routing policies. 
Addressing such challenges in a dynamic environment is a key motivation for adopting online learning approaches for LLM routing, as they offer the ability to continuously learn and optimize the routing policy in real time.
The online algorithms adopted in prior work can be categorized into three classes: multi-armed bandits \cite{MetaLLM, C2MAB-V, LLM Bandit}, contextual bandits \cite{MixLLM}, and reinforcement learning \cite{PickLLM}.

Toward building a practical routing system to fit the various requests, multiple challenges should be addressed simultaneously. 
However, we notice that there was little effort at jointly solving the challenges of adaptivity and weak supervisions, even if the community have already acquired huge progress in respective directions.
To our best knowledge, \cite{MixLLM} is the only attempt to address adaptivity and pointwise feedback (e.g., like/dislike) at the same time.
Therefore, the current paper targets on investigating LLM routing under the stochastic bandit setting with a weak supervision of pairwise preference feedback (e.g., reply A is better than reply B).
The advantages of the project is threefold:
First, we introduce the contextual dueling bandit algorithm \cite{FGTS.CDB} as the core module.
It naturally combines weak supervision (i.e., the dueling feedback) and adaptive learning (i.e., the bandit algorithm) in the algorithm input and the design of the learning procedure.
Its introduction provides the community with broader methodological choices for future research.
Second, it is a theoretically justified method that offers a clear explanation of how binary feedback is connected to the utility function that defines the model's performance, which is a complex function of user satisfaction, model expertise, and model cost.
Third, it provides a platform for us to investigate what makes it work and what makes it fail, so that we can realize it to be the first practical LLM router that does not require high-quality annotations and is robust to dynamically changing environments.

The paper’s contributions are summarized as follows.
\begin{itemize}
    \item We propose Category-Calibrated Fine-Tuning (CCFT), a generic embedding method to encode an LLM’s expertise.
    The feature function constructed by CCFT allows us to build the first trainable contextual dueling learner in LLM routing.
    \item Strong evidence of efficacy of the proposed method is observed from experimenting two real-world datasets, RouterBench \cite{RouterBench} and Mix-Instruct \cite{Mix-Instruct}.
    All four implementations of CCFT are tested and compared to each other.
    The curves of cumulative regret demonstrate the behavior of the proposed method converging to the optimal strategy that chooses the best matching model for each question.
    \item The proposed method also demonstrate merits of robust generalization to unseen benchmark and performance-cost balance.
    \item In the experiments, several common practices of LLM, including prompting, context fine-tuning, open-sourced and block-box text embedding models, are integrated with the proposed method, accumulating substantial knowledge and skills of addressing LLM routing.
\end{itemize}





























==> iclr2026/94_failure_examples_250924.tex <==

\subsection{The Failure of Naive Implementations}
\label{sec:failure_cases_2}
This subsection demonstrates the practical challenge of a carefully designed feature function.
We chose five topics\footnote{They are abstract algebra, anatomy, astronomy, international law, and machine learning.} from MMLU. 
Questions \mycmt{(unify question vs query)} are sampled to form two disjoint offline learning and online testing sets.
We assume there are five LLMs, each with expertise in one of the topics.
% We tried two ways to generate the model embeddings $\rho_k$.
\fix
We tried two ways to generate the model embeddings $a_k$\footnote{To avoid a disconnection from the previous section, we use $a_k$ to both index an LLM (as we did previously) and denote the LLM's embedding (as we will elaborate next). (depending on the context)}.
Each way takes the offline questions to build five model embeddings.
% Each way takes the offline questions of one topic and is repeated\mycmt{(?)} five times to build five model embeddings.
In the first way, we encode the model description via OpenAI's \texttt{text-embedding-3-large}, where the model description is the combination of our handcrafted prompt with offline questions (Listing~\ref{code_snippet:prompt_mmlu} in Appendix~\ref{sec:prompts}).
In the second way, we first generate offline question embeddings of a topic using \texttt{text-embedding-3-large} and then take their average as the model embedding. 
The intuition behind both approaches is to represent a model using the sample questions it excels at.
It is rather simple to generate a question embedding $x$, as we simply feed the question string into \texttt{text-embedding-3-large}.
We tested the Hadamard product (element-wise multiplication) $\phi(x, a) = x * a$ with normalization and vector addition (element-wise addition) $\phi(x, a) = x + a$ with normalization to construct $\phi$ and keep the first one based on the experimental outcomes.

% \begin{figure}[htbp]
%     \centering
    
%     % Subfigure (a)
%     \begin{subfigure}[t]{0.45\textwidth}
%         \includegraphics[width=\linewidth]{plots/mmlu_set2_figure_1.pdf}
%         \caption{FGTS.CDB with failed model embeddings}
%         \label{fig:failure_exs_a}
%     \end{subfigure}
%     % \hfill
%     % Subfigure (b)
%     \begin{subfigure}[t]{0.45\textwidth}
%         \includegraphics[width=\linewidth]{plots/mmlu_set2_figure_2.pdf}
%         \caption{A successful example}
%         \label{fig:failure_exs_b}
%     \end{subfigure}

%     \caption{Failure vs Success Learning in Contextual Dueling Bandits (FGTS.CDB). Cumulative regret is shown across evaluation rounds. A flat slope indicates good learning progress, as it reflects a slow accumulation of regret.}
%     \label{fig:failure_exs_old}
% \end{figure}
% \bcmt{(Figure creation: \url{https://chatgpt.com/c/68be7116-5bb0-8324-bdea-ab37025f7b70})}
\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-4mm}
\begin{minipage}{0.45\textwidth}
    \begin{center}
    \includegraphics[width=1.\linewidth]{plots/mmlu_set2_figure_0_main.pdf}
    \vspace{-8mm}
    \end{center}
    \caption{Failed versus successful examples.}
    \label{fig:failure_exs_2}
\end{minipage}
\vspace{-4mm}
\end{wrapfigure}
From Figure\ref{fig:failure_exs}, we see that the slopes of the orange and blue curves\mycmt{(?)} almost do not change with rounds. 
This means the regret keeps accumulating, and hence the learning does not progress a lot.
In contrast, the slope of the red curve reduces as the rounds increase. 
This small cumulative regret reflects that the learning agent is making fewer and fewer mispredictions and converging the behavior toward the best routing strategy. 
In the next subsection, we propose a generic strategy to construct model embeddings achieving a similar behavior to the red curve\mycmt{(?)} and then test its realizations on real-world datasets in experiments.


==> iclr2026/95_main_ver2_250921.tex <==



\section{Introduction}
\label{sec:intro}
The potential of LLMs is so large that it almost becomes a necessary part of daily life, with applications from office assistance, fashion/dining suggestions, to entertainment.
LLM routing refers to a problem of dynamically selecting the most suitable LLM from a set of candidates for each query from a sequence of questions.
Before the emergence of a universally dominant and affordable foundation model, routing is important as a suitable LLM matches the user traits, the model expertise, and the cost.
To balance these three key factors, cascading algorithms FrugalGPT \citep{chen2024frugalgpt} and AutoMix \citep{AggarwalMAPMZGR24} were first proposed.
The idea is to query a cheap model first and advance the query to a more expensive model if the current reply is likely to fail the user’s expectation.

A drawback of cascading is the accumulated cost and latency caused by a series of calls to multiple LLM candidates to obtain the final reply to output.
To avoid this, supervised routing methods \citep{shnitzer2023llmrouting, lu2024zooter, ding2024hybridllm, hu2024routerbench, srivatsa2024harnessing} were proposed.
In general, a supervised router reduces the latency by applying a classification or a regression prediction before the LLM query.
The supervised approach has evolved into branches. 
A branch studied ensembles \citep{jiang2023mixinst_blender, maurya-etal-2025-selectllm, zhang2025avengers, zhang2025avengerspro}, which allows the agent to select a subset or fuse answers. 
Another branch exercised cost-aware model assignment \citep{sakota2024forc, hu2024routerbench, liu2024optllm} to balance the cost and performance.
There are also works that combine representation learning \citep{feng2025graphrouter, zhuang2025embedllm} to strengthen the user and model’s semantic information before training.

For supervised routing methods, having abundant real-valued annotations with high-quality label information is critical for successful classification or regression training.
Unfortunately, such a requirement is often unrealistic in the context of LLM routing.
In some cases, users are either reluctant or unmotivated to provide feedback. 
They may also be unable to quantify their satisfaction, especially when dealing with open-ended questions or when they lack the ability to verify the correctness of the LLM's response.
To ease the annotation burden, some efforts focused on weak supervision \citep{sugiyama2022weak, chiang2025unified}, which only collect binary feedback such as like/dislike or pairwise comparison \citep{ong2025routellm, zhao2024eagle, wang2025mixllm}.
The advantage is that one-click feedback is user-friendly, and it is more confident to say reply A is better than B than to assign reply A a score out of ten.
The reason that makes a weakly supervised approach appealing is that, as shown by the referred papers, the binary feedback can be translated into a model ranking or an estimate of the labeling function. 

In addition to the challenge of annotation, adaptivity remains a key challenge to be addressed in developing a usable routing system.
Shifts in query distributions, such as changes in trending topics like fashion or temporal variations between work hours and leisure time, introduce non-stationary conditions. 
Moreover, new LLMs and benchmarks are continuously introduced, resulting in a constantly evolving environment for routing.
These evolving conditions often exceed the capacity of static, supervised learning-based routing policies. 
Addressing such challenges in a dynamic environment is a key motivation for adopting online learning approaches for LLM routing, as they offer the ability to continuously learn and optimize the routing policy in real time.
The online algorithms adopted in prior work can be categorized into three classes: multi-armed bandits \citep{nguyen2024metallm, dai2024C2MAB-V, li2025llmbandit}, contextual bandits \citep{wang2025mixllm}, and reinforcement learning \citep{sikeridis2025pickllm}.

To build a practical routing system to fit the various requests, multiple challenges should be addressed simultaneously. 
However, we notice that there was little effort at jointly solving the challenges of adaptivity and weak supervision, even if the community has already made huge progress in respective directions.
To our best knowledge, \cite{wang2025mixllm} is the only attempt to address adaptivity and pointwise feedback (e.g., like/dislike) at the same time.
Therefore, this paper focuses on investigating LLM routing under a stochastic bandit setting, which captures the dynamics of a changing environment, and operates under weak supervision in the form of pairwise preference feedback (e.g., reply A is preferred over reply B)\footnote{\bcmt{[CK] Let's fix a term. Reply or response?}}.
The advantages of the project are threefold:
First, we introduce the contextual dueling bandit algorithm FGTS.CDB \citep{li2024fgtscdb} as the core module.
It naturally combines weak supervision (i.e., the dueling feedback) and adaptive learning (i.e., the bandit algorithm) in the algorithm input and the design of the learning procedure.
Its introduction provides the community with broader methodological choices for future research.
Second, it is a theoretically justified method that offers a clear explanation of how binary feedback is connected to the utility function that defines the model's performance, which is a complex function of user satisfaction, model expertise, and model cost.
Third, it provides a platform for us to investigate what makes it work and what makes it fail, so that we can realize it to be the first\mycmt{(?)} practical LLM router that does not require high-quality annotations and is robust to dynamically changing environments.

The paper’s contributions are summarized as follows.
\begin{itemize}
    \item We propose Category-Calibrated Fine-Tuning (CCFT), a generic embedding method to encode an LLM’s expertise.
    The feature function constructed by CCFT allows us to build the first trainable contextual dueling learner in LLM routing.
    \item Strong evidence of the efficacy of the proposed method is observed from experimenting with two real-world datasets, RouterBench \citep{hu2024routerbench} and MixInstruct \citep{jiang2023mixinst_blender}.
    All four implementations of CCFT are tested and compared to each other.
    The curves of cumulative regret demonstrate the behavior of the proposed method converging to the optimal strategy that chooses the best matching model for each question.
    \item The proposed methods also demonstrate the merits of robust generalization to an unseen benchmark and performance-cost balance.
    \item In the experiments, several common practices of LLM, including prompting, context fine-tuning, open-sourced and block-box text embedding models, are integrated with the proposed method, accumulating substantial knowledge and skills of addressing LLM routing.
\end{itemize}




\section{Related Work}

\subsection{LLM Routing}
\label{sec:related_routing}
\citet{ong2025routellm}

\subsection{Contextual Dueling Bandits and Feel-Good Thompson Sampling}
\label{sec:bandits}
Research on contextual dueling bandits has advanced along several directions. \cite{kumagai2017continuousdueling} analyzed dueling bandits with a continuous action space and, under strong convexity and smoothness, established dimension-free regret guarantees. Building on preference models, \cite{bengs2022stochasticcontextual} introduced the CoLSTIM algorithm for stochastic contextual dueling bandits under linear stochastic transitivity, providing learning guarantees tailored to this structure. Recently, \cite{di2024varianceaware} proposed VACDB, an action-elimination-based method that achieves tighter, variance-dependent regret bounds for contextual settings.

Feel-Good Thompson Sampling (FGTS) was proposed to reconcile Thompson sampling’s strong empirical performance with frequentist-style guarantees \citep{zhang2022fgts}. \cite{fan2023powerfgts} offered a unified analysis framework showing how FGTS yields robust guarantees across several linear contextual bandit variants. The FGTS idea has also been extended to reinforcement learning, e.g., Model-based Optimistic Posterior Sampling (MOPS) for Markov decision processes \citep{agarwal2022modelbasedops}. To our best knowledge, our work is the first to apply FGTS to LLM routing, connecting preference-based bandit principles with practical model-selection pipelines.


\section{Background}
\label{sec:background}

\subsection{Feel-Good Thompson Sampling for Contextual Dueling Bandits}
\rcmt{Need a section level symbol refinement.}
The contextual dueling bandit problem can be seen as a repeated game between a bandit algorithm and an environment for T rounds. 
In each round $t = 1, 2, \ldots T$, the algorithm observes a contextual vector $x_t$ from the environment.
% In each round $t = 1, 2, \ldots T$, the algorithm observe a contextual vector $x_t$ representing the query from the environment.
Then, the algorithm selects two actions $a^1_t, a^2_t \in \mathcal{A} = \{k\}_{k=1}^{K}$\mycmt{(resp. $\{a_k\}_{k=1}^{K}$)} as responses.
After presenting the responses, the algorithm observes a preference feedback $y_t$.
The performance of the algorithm is measured by its cumulative regret 
\eqary{
    \operatorname{Regret}(T) 
    := \sum_{t=1}^{T} \left[ r^{*}(x_t, a_t^{*}) - \frac{r^{*}(x_t, a_t^{1}) + r^{*}(x_t, a_t^{2})}{2} \right],
    \num\label{eq:regret}
}
where $r^{*}(x, a)$ is the utility function and $a_t^{*} = \arg\max_{a \in \mathcal{A}} r^{*}(x_t, a)$ is the best action for input $x_t$.

The setting fits seamlessly to the LLM routing problem studied in this paper if we view $x_t$ as the query embedding,
% that encodes query semantics and user traits, 
$a^1_t$ and $a^2_t$ as two LLMs, $y_t$ as the preference feedback, and the $r^{*}(x, a)$ as the function balancing the user satisfaction and model score\footnote{The model score is calculated from the LLM performance, cost, latency, and other interested factors.} that we want to optimize.
The connection between the weak supervision of preference feedback $y$ and the ideal supervision provided by $r^{*}(x, a)$ is captured by the Bradley--Terry--Luce (BTL) model~\citep{hunter2004btl, luce2005btl}:
Given query $x$ and two LLMs $a^1$ and $a^2$, the probability of observing $a^1$ is preferred over $a^2$ (i.e., $y=1$) is
\eqary{
    \mathbb{P}(y = 1 \mid x, a^1, a^2) 
    = 
    % \frac{\exp(r^{*}(x, a^1))}{\exp(r^{*}(x, a^1)) + \exp(r^{*}(x, a^2))}
    % = 
    \exp\big(-\sigma(r^{*}(x, a^1) - r^{*}(x, a^2))\big),
}
where $\sigma(z) = \log(1 + \exp(-z))$\footnote{
A more general setting accepting more than two candidates is called the Plackett-Luce (PL) model \citep{pmlr-v32-soufiani14, pmlr-v48-khetan16, ren2018pacranking}.
}.

\begin{algorithm}
\caption{FGTS.CDB}\label{alg:fgts-cdb}
\begin{algorithmic}[1]
\State Given action space $\mathcal{A}$ and hyperparameters $\eta, \mu$. Initialize $S_0 = \varnothing$.
\For{$t = 1, \ldots, T$}
  \State Receive query $x_t$.
  \For{$j = 1, 2$}
    \State Sample model parameter $\theta_t^{j}$ from the posterior distribution: 
    \eqary{
        p^j(\theta \mid S_{t-1}) 
        \propto 
        \exp\left( -\sum_{i=1}^{t-1} L^j(\theta, x_i, a_i^1, a_i^2, y_i) \right) p_0(\theta)
    }
    % $p^{j}(\,\cdot \mid S_{t-1})$, defined in (4.1).
    \State Select LLM $a_t^{j} = \arg\max_{a \in \mathcal{A}}\; \langle \theta_t^{j}, \,\phi(x_t,a) \rangle$ to generate the response.
  \EndFor
  \State Receive preference feedback $y_t$.
  \State Update history $S_t \leftarrow S_{t-1} \cup \{(x_t, a_t^{1}, a_t^{2}, y_t)\}$.
\EndFor
\end{algorithmic}
\end{algorithm}
Assuming the linear reward model $r^{*}(x, a) = \langle \theta^{*}, \phi(x, a) \rangle$, \cite{li2024fgtscdb} proposed Algorithm~\ref{alg:fgts-cdb} and proved that it achieves $\mathbb{E}[\operatorname{Regret}(T)] = \widetilde{\mathcal{O}}(d\sqrt{T})$, where $d$ is the dimension $\theta$. 
FGTS.CDB learns the LLM selection strategies, $\theta^{1}_t$ and $\theta^{2}_t$, in an online fashion.
Its success hinges on the posterior $p^j(\theta \mid S_{t-1})$ defined by the likelihood function
\eqary{
    L^j(\theta, x, a^1, a^2, y) 
    = 
    \eta \, \sigma\big(y \langle \theta, \phi(x, a^1) - \phi(x, a^2) \rangle \big) - \mu \max_{\tilde{a} \in \mathcal{A}} \langle \theta, \phi(x, \tilde{a}) - \phi(x, a^{3-j}) \rangle.
}
The intuition behind $L^{j}(\cdot)$ is as follows: if $\theta$ aligns well with the preference feedback $y$, that is, when $y \langle \theta, \phi(x, a^1) - \phi(x, a^2) \rangle$ is positive and large, then $\theta$ is more likely to be chosen.
The second term in the likelihood function serves as a ``feel-good'' component, encouraging the selection of a $\theta$ that outperforms past selections made by the other selection strategy\footnote{Specifically, note that, $a^{3-j} = a^2$ for $j=1$ and $a^{3-j} = a^1$ for $j=2$.}. 
As time $t$ progresses, the observation history $S_t$ accumulates, allowing FGTS to dynamically adjust its samples $\theta^{1}_{t+1}$ and $\theta^{2}_{t+1}$ accordingly.
In an evolving environment, any changes are reflected in $S_t$, and adaptivity is inherently ensured by the bandit algorithm.

Being theoretically oriented, \cite{li2024fgtscdb} assumes that the feature function $\phi(x, a)$ is given and perfect. 
However, this assumption generally does not hold in real-world applications.
In Section~\ref{sec:failure_cases}, we demonstrate how an imperfect $\phi(x, a)$ can hinder learning and highlight a key obstacle in applying FGTS.CDB to the routing problem.
Subsequently, in Section~\ref{sec:proposed_model_emb}, we introduce our method for constructing a feature function that enables FGTS.CDB, with the aforementioned merits, to function effectively in practical LLM routing scenarios.


% \subsection{Context Contrastive Fine-Tuning}
% \rcmt{Here or Appendix?}


% \subsection{Materials}

% \noindent\textbf{Stochastic Preference Model.} 
% In this work, we assume that the preference $y_t$ follows a Bernoulli distribution 
% according to the Bradley--Terry--Luce (BTL) model~\cite{Hunter2004,Luce2005}: 
% Given context $x_t$ and responses $a_t^1, a_t^2$, 
% the probability of $a_t^1$ being preferred over $a_t^2$ is
% \eqary{
%     \mathbb{P}(y_t = 1 \mid x_t, a_t^1, a_t^2) 
%     = 
%     \frac{\exp(r^{*}(x_t, a_t^1))}{\exp(r^{*}(x_t, a_t^1)) + \exp(r^{*}(x_t, a_t^2))}
%     = 
%     \exp\big(-\sigma(r^{*}(x_t, a_t^1) - r^{*}(x_t, a_t^2))\big),
% }
% where $\sigma(z) = \log(1 + \exp(-z))$\footnote{
% A more general setting accepting more than two candidates is called the Plackett-Luce (PL) model \cite{Soufiani et al., 2014; Khetan & Oh, 2016; Ren et al., 2018}.
% }.

% \noindent\textbf{Learning Objective.} 
% The goal is to minimize the cumulative average regret:
% \eqary{
%     \operatorname{Regret}(T) 
%     := \sum_{t=1}^{T} \left[ r^{*}(x_t, a_t^{*}) - \frac{r^{*}(x_t, a_t^{1}) + r^{*}(x_t, a_t^{2})}{2} \right],
% }
% where $a_t^{*} = \arg\max_{a \in \mathcal{A}} r^{*}(x_t, a)$ is the optimal LLM for question $x_t$.




\section{A Generic Representation Learning Method}
\label{sec:generic_method}

\subsection{The Failure of Naive Implementations}
\label{sec:failure_cases}
This subsection demonstrates the practical challenge of a carefully designed feature function.
We chose five topics\footnote{They are abstract algebra, anatomy, astronomy, international law, and machine learning.} from MMLU. 
Questions are sampled to form the offline learning and online testing sets.
We assume there are five LLMs, each with expertise in one of the topics.
We tried two ways to generate the model embeddings $\rho_k$.
\mycmt{(revise?) We use $a_k$ to both index an LLM and denote its model embedding; this would simplify the symbols.}
\rcmt{(revise?) Replace $\rho_k$ with $a_k$.}
Each way takes the offline questions of one topic and is repeated\mycmt{(?)} five times to build five model embeddings.
In the first way, we encode the model description via OpenAI's \texttt{text-embedding-3-large}, where the model description is the combination of our handcrafted prompt with offline questions.
In the second way, we first generate offline question embeddings using \texttt{text-embedding-3-large} and then take their average as the model embedding of the corresponding topic. 
The intuition behind both approaches is to represent a model using the sample questions it excels at.
It is rather simple to generate a question embedding $x$, as we simply feed the question string into \texttt{text-embedding-3-large}.
We tested the Hadamard product (element-wise multiplication) $\phi(x, a) = x * a$\mycmt{(integrate with $\rho_k$? Or simply use text to refer $a_k$ as both index and embedding?)} with normalization and vector addition (element-wise addition) $\phi(x, a) = x + a$ with normalization to construct $\phi$ and keep the first one based on the experimental outcomes.

\begin{figure}[htbp]
    \centering
    
    % Subfigure (a)
    \begin{subfigure}[t]{0.45\textwidth}
        \includegraphics[width=\linewidth]{plots/mmlu_set2_figure_1.pdf}
        \caption{FGTS.CDB with failed model embeddings}
        \label{fig:failure_exs_a}
    \end{subfigure}
    % \hfill
    % Subfigure (b)
    \begin{subfigure}[t]{0.45\textwidth}
        \includegraphics[width=\linewidth]{plots/mmlu_set2_figure_2.pdf}
        \caption{A successful example}
        \label{fig:failure_exs_b}
    \end{subfigure}

    \caption{Failure vs Success Learning in Contextual Dueling Bandits (FGTS.CDB). Cumulative regret is shown across evaluation rounds. A flat slope indicates good learning progress, as it reflects a slow accumulation of regret.}
    \label{fig:failure_exs}
\end{figure}
% \bcmt{(Figure creation: \url{https://chatgpt.com/c/68be7116-5bb0-8324-bdea-ab37025f7b70})}
From Figure\ref{fig:failure_exs_a}, we see that the slope almost does not change with rounds. 
This means the regret keeps accumulating, and hence the learning does not progress a lot.
In contrast, the slope of the curve in Figure\ref{fig:failure_exs_b} reduces as the rounds increase. 
This small cumulative regret reflects that the learning agent is making fewer and fewer mispredictions and converging the behavior toward the best routing strategy. 
In the next subsection, we propose a generic method to construct model embeddings achieving a similar behavior to Figure\ref{fig:failure_exs_b} and then test its realizations on real-world datasets in experiments.



\subsection{The Proposed Method}
\label{sec:proposed_model_emb}

Note that by design, $\phi(x_t, a)$ combines the information from the user side, $x_t$, and the information from the LLM side, $a$.
Since the text models we selected are well-recognized sentence encoders, the failure cases discussed in Section~\ref{sec:failure_cases} are most likely due to careless design of the model embeddings.
% Therefore, it is imperative to ensure that $a_k$ accurately captures the characteristics of the corresponding LLM $k$.
Therefore, it is imperative to ensure that $a_k$\mycmt{(resp. $\rho_{a}$)} accurately captures the connection between the potential-to-see questions and the expertise of LLM $k$\mycmt{(resp. $a$)}.
In this section, we introduce \emph{Category-Calibrated Fine-Tuning (CCFT)}, a generic method for learning $a$ via contrastive fine-tuning combined with categorical weighting.


% The failure cases in Section~\ref{sec:failure_cases} show that a careful design of the model embedding $a$ is needed.
% In this section, we propose Category-Calibrated Fine-Tuning (CCFT), a generic method to train $a$ via contrastive fine-tuning and categorical weighting.
% Note that by design, $\phi(x_t, a)$ combines the information from the user side, $x_t$, and the information from the LLM side, $a$.  
% Therefore, it is imperative to make sure that $a_k$ captures the characteristics of LLM $k$.
Suppose the questions can be divided into $M$ categories\footnote{A category can refer to a topic, a benchmark, or query type, depending on the dataset.}, such as fashion, opinion, history, biology, finance, and so on.
The 3D t-SNE plot of the failure examples in Figure~\ref{fig:tsne-3d} shows that the text model tends to cluster questions from the same category.
It provides contrastive fine-tuning a good starting point.
Thus, we fine-tune the text model using a small offline question set that is disjoint from the online testing set.
Then, for each category $m$, we compute the category embedding $\xi_m$ by averaging the embeddings of offline questions belonging to that category, as generated by the fine-tuned text model. 
Note that the category embedding $\xi_m$ is not the model embedding $\rho_k$, for which an additional step is required, as described next.

To capture the unique characteristics of each LLM, we assume that every LLM is associated with a distinct Kiviat diagram, representing its areas of expertise.
Under this assumption, a natural approach is to compute a weighted combination of the category embeddings, where the weights are derived from the LLM’s scores on its Kiviat diagram. We refer to this mechanism as ``categorical weighting''.
In particular, we propose the following four weighting methods.
Denote $M$ category embeddings $(\xi_1, \xi_2, \ldots, \xi_M) := \xi$.
For each LLM $a_k$, let $(s_{k,1}, s_{k,2}, \ldots, s_{k,M})^{\top} := s_k$ be the score vector over the categories.
The first weighting method, coined ``\texttt{perf}'', defines the model embedding of $a_k$ as
\eqary{
    \rho_k = \xi \operatorname{softmax}(s_k) , 
    \num\label{eq:def_perf}
}
where $s_{k,m}$ is the model performance on category $m$.
If the score $s_{k,m}$ is a function of model performance and model cost, we coin the resulting $\rho_k$ ``\texttt{perf\_cost}''.
Note that \texttt{perf} and \texttt{perf\_cost} take all score values into account.
In reality, a common scenario involves a few strong models that specialize in different categories, alongside several weaker models that perform comparably within specific domains.
In such a case, we could weight an LLM only on categories it is good at, and leave the other categories handled by other LLMs.
Formalizing this idea, we propose ``\texttt{excel\_perf\_cost}'' as
\eqary{
    \rho_k = \xi \operatorname{softmax}\left(\operatorname{top}^{(\tau)}(s_k) \right),
    \num\label{eq:def_excel_perf_cost}
}
and ``\texttt{excel\_mask}'' as
\eqary{
    \rho_k = \xi \frac{\operatorname{mask}^{(\tau)}(s_k)}{\tau}.
    \num\label{eq:def_excel_mask}
}
Let $\tau \in [K]$, and let $s_{(\tau),m}$ denote the $\tau$-th largest value in $\{ s_{1,m}, s_{2,m}, \ldots, s_{K,m} \}$\footnote{Sorting $\{ s_{1,m}, s_{2,m}, \ldots, s_{K,m} \}$ results in $s_{(1),m} \geq s_{(2),m} \geq \ldots \geq s_{(K),m}$, and $s_{(\tau),m}$ will be located at the $\tau$-th position.}.
Function $\operatorname{top}^{(\tau)}(s_k)$ produces a real-valued vector with $m$-th entry $\operatorname{top}^{(\tau)}(s_k)_{m} = s_{k,m} \mathbf{1}[s_{k,m} \geq s_{(\tau),m}]$.
Similarly, function $\operatorname{mask}^{(\tau)}(s_k)$ produces a binary vector with $m$-th entry $\operatorname{mask}^{(\tau)}(s_k)_{m} = \mathbf{1}[s_{k,m} \geq s_{(\tau),m}]$.
% Let $\tau \in [M]$, and let $s_{k,(\tau)}$ denote the $\tau$-th largest value in $s_k$. 
% Function $\operatorname{top}^{(\tau)}(s_k)$ produces a real-valued vector with $m$-th entry
% \eqary{
%     \operatorname{top}^{(\tau)}(s_k)_{m} = s_{k,m} \mathbf{1}[s_{k,m} \geq s_{(\tau),m}] = 
%     \begin{cases}
%         s_{k,m} & \text{if } s_{k,m} \geq s_{(\tau),m},\\
%         0 & \text{otherwise.}
%     \end{cases}
% }
% Function $\operatorname{mask}^{(\tau)}(s_k)$ produces a binary vector with $m$-th entry
% \eqary{
%     \operatorname{mask}^{(\tau)}(s_k)_{m} = \mathbf{1}[s_{k,m} \geq s_{(\tau),m}] = 
%     \begin{cases}
%         1 & \text{if } s_{k,m} \geq s_{(\tau),m},\\
%         0 & \text{otherwise.}
%     \end{cases}
% }

Now, we have three ways of computing an LLM embedding.
The main idea behind these mechanisms is that the scores reflect the expertise of an LLM over the categories, the category embeddings abstract the potential-to-see questions, and the definitions $\rho_k$ show how we model the connection of these two key factors.


\subsubsection{Categorical Weighting without Scores}

Note that the weighting mechanisms (\ref{eq:def_perf}), (\ref{eq:def_excel_perf_cost}), and (\ref{eq:def_excel_mask}) require score information, which might not always be the case.
Next, we show that we can still perform a way of categorical weighting under a mild condition.

Suppose the label of a question records its best matching LLM.
Thus, we use $f_{km}$ to denote the proportion\footnote{\bcmt{A future potential: A new project of LLM + label proportion?}} of label $k$ in category $m$.
We next assume the offline data is generated as follows:
From each category $m$, a set of questions $\mathcal{Q}_m$ of size $n$ is sampled.
The offline data is $\{ \mathcal{G}_k \}_{k=1}^{K}$, formed by regrouping $\{ \mathcal{Q}_m \}_{m=1}^{M}$ according to the labels.
Given $\mathcal{G}_k$, we propose to compute the model embedding of $a_k$ by averaging over the question embeddings: Let $h$ be an embedding function and $q \in \mathcal{G}_k$ be a question. For each LLM $a_k$,
\eqary{
    % \rho_k = \frac{\sum_{q \in \mathcal{G}_k} h(q)}{|\mathcal{G}_k|}.
    \rho_k = \sum_{q \in \mathcal{G}_k} h(q) / |\mathcal{G}_k|.
    \num\label{eq:def_mix_inst}
}
The following proposition justifies the proposed mechanism.
\begin{proposition}
    % Let $h$ be an embedding function and 
    Let $\mathcal{Q}_m$ be the set of questions of size $n$ uniformly sampled from category $m$.
    Denote the proportion of label $k$ in category $m$ as $f_{km}$\footnote{ W.l.o.g., we assume $f_{km} n$ is an integer for all $k, m$.}.
    Let $Q_m$ be a random variable of questions of category $m$ sampled uniformly at random and $\mathbb{E}[h(Q_m)]$ be the expected question embedding.
    Suppose $\{ \mathcal{G}_k \}_{k=1}^{K} \}$ are given, where $\mathcal{G}_k$ gathers all questions labeled $k$ in $\{ \mathcal{Q}_m \}_{m=1}^{M}$.
    For each $k \in [K]$, the average embedding calculated from $\mathcal{G}_k$ is an unbiased estimate for
    \eqary{
        \sum_{m=1}^{M} \frac{f_{km}}{\sum_{j=1}^{M} f_{kj}} \mathbb{E}[h(Q_m)].
    }
\end{proposition}
\begin{proof}
    Let $k$ be fixed.
    % Let $q$ be a question.
    Note that the size of $\mathcal{G}_k$ is $\sum_{j=1}^{M} f_{kj} n$.
    Then,
    \eqary{
        \frac{\sum_{q \in \mathcal{G}_k} h(q)}{|\mathcal{G}_k|}
        =\ &
        \frac{\sum_{m=1}^{M} \sum_{q \in \mathcal{Q}_m} h(q)}{\sum_{j=1}^{m} f_{kj} n} 
        =\ 
        \sum_{m=1}^{M} \frac{f_{km} n}{\sum_{j=1}^{M} f_{kj} n} \frac{\sum_{q \in \mathcal{Q}_m} h(q)}{f_{km} n}.
    }
    Hence, we have the proposition by noting that $\frac{\sum_{q \in \mathcal{Q}_m} h(q)}{f_{km} n}$ is an unbiased estimation for $\mathbb{E}[h(Q_m)]$.
\end{proof}

The proposition shows that, even if there is no score information available, averaging over question embeddings still offers a way of categorical weighting in terms of label proportions: the weighting coefficients are $ \frac{f_{km}}{\sum_{j=1}^{M} f_{kj}}, m=1, \ldots, M$.
Note that a constraint is the constant $n$ over categories.
The constraint can be relaxed if we know the number of samples from each category.
Furthermore, when a pool of pairwise comparison results is gathered, one can build a rank over LLMs to determine the best matching model. 
Therefore, the $\{ \mathcal{G}_k \}$ setting and the proposed model embedding mechanism in this section fit naturally into many industrial applications.












\section{Experiments}
\label{sec:experiments}
\mycmt{(FGTS.CDB and its SGLD module)}
We implemented FGTS.CDB shown in Algorithm~\ref{alg:fgts-cdb}. 
Sampling from the posterior $p^j(\theta \mid S_{t-1})$ in Step 5 is implemented by the Stochastic Gradient Langevin Dynamics (SGLD) algorithm \citep{welling2011GDLD}.

\mycmt{(Text embedding models)}
Four text embedding models are chosen to generate embeddings for queries.
They are: OpenAI's \texttt{text-embedding-3-large} \citep{openai-text-embedding-3-large}, \texttt{all-MiniLM-L6-v2} \citep{sentence-transformers-all-MiniLM-L6-v2}, \texttt{all-mpnet-base-v2} \citep{sentence-transformers-all-mpnet-base-v2}, and \texttt{intfloat/e5-base} \citep{wang2022e5}.
In this paper, we refer to the models as \texttt{OpenAItext}, \texttt{MiniLM}, \texttt{mpnet}, and \texttt{e5b}, respectively.
\texttt{OpenAItext} serves as a strong and general-purpose embedding model.
We compare its embeddings with those generated by the fine-tuned \texttt{MiniLM}, \texttt{mpnet}, and \texttt{e5b} models to examine their impact on the feature function $\phi(x, a)$ derived from a text model.

\mycmt{(Contrastive fine-tuning)}
The fine-tuning for an open-sourced text embedding model is implemented by contrastive learning \citep{Khosla20SCL, Nils2019sentenceBERT}. 
We first build similar/dissimilar query pairs according to their source category or benchmark.
Then, the cosine-similarity loss is used to fine-tune the model.
For instance, \texttt{eb5\_E4} means that \texttt{eb5} is fine-tuned for four epochs, and \texttt{mpnet\_E2} represents \texttt{mpnet} fine-tuned for two epochs. 

\mycmt{(Prompting OpenAI's \texttt{text-embedding-3-large})}

\subsection{RouterBench}
\label{sec:exp_routerb}
RouterBench \citep{hu2024routerbench} is a comprehensive benchmark designed for evaluating LLM routing methods. 
It provides over 405k precomputed inference outputs from eleven diverse LLMs across seven tasks (MMLU, MT-Bench, MBPP, HellaSwag, Winogrande, GSM8K, ARC). 
The dataset includes detailed performance and cost metadata, enabling systematic analysis of routing strategies.
The metadata, organized into a table in \cite{hu2024routerbench} is included as Table~\ref{table:Table_1_routerb} in Appendix~\ref{sec:more_categorical_weighting}.

Next, we describe how to use the metadata and the queries in each benchmark to construct the model embedding $\rho_k$ for LLM $a_k$.
The learning process is divided into two phases: an offline fine-tuning phase, during which the model embeddings are learned, and an online testing phase, where a realization of FGTS.CDB is evaluated through a sequence of queries. 
To apply the proposed method, we need to compute $s_k$ and $\xi$.
Each benchmark $m$ is treated as a distinct category. 
To compute the corresponding category embedding $\xi_m$, we apply a text embedding model to five queries sampled from benchmark $m$, and then take the average of their embeddings.
\mycmt{(compare; distinctive) We only need 35 queries vs. MixLLM needs 30\% of the data.}
These sampled queries are excluded from the online learning phase to prevent data leakage.
Suppose \texttt{e5b\_E4} is applied to generate the embedding, then we obtain $\xi^{(\texttt{e5b\_E4})} = \left( \xi_{\textrm{MMLU}}^{(\texttt{e5b\_E4})}, \xi_{\textrm{MT-Bench}}^{(\texttt{e5b\_E4})}, \ldots, \xi_{\textrm{ARC}}^{(\texttt{e5b\_E4})} \right)$.

\begin{table*}[htbp]
\centering
\caption{Scores of \texttt{Perf\_cost}, \texttt{Excel\_perf\_cost}, and \texttt{Excel\_mask}}
\label{table:weighting}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccccccccccccccccccccccc}
\toprule
\textbf{LLM} & 
\multicolumn{3}{c}{\textbf{MMLU}} & 
\multicolumn{3}{c}{\textbf{MT-Bench}} & 
\multicolumn{3}{c}{\textbf{MBPP}} & 
\multicolumn{3}{c}{\textbf{HellaSwag}} & 
\multicolumn{3}{c}{\textbf{Winogrande}} & 
\multicolumn{3}{c}{\textbf{GSM8k}} & 
\multicolumn{3}{c}{\textbf{ARC}} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}
\cmidrule(lr){11-13}
\cmidrule(lr){14-16}
\cmidrule(lr){17-19}
\cmidrule(lr){20-22}
& (i) & (ii) & (iii) 
& (i) & (ii) & (iii) 
& (i) & (ii) & (iii) 
& (i) & (ii) & (iii) 
& (i) & (ii) & (iii) 
& (i) & (ii) & (iii) 
& (i) & (ii) & (iii) \\
% & (\ref{eq:def_perf}) & (\ref{eq:def_excel_perf_cost}) & (\ref{eq:def_excel_mask}) 
% & (\ref{eq:def_perf}) & (\ref{eq:def_excel_perf_cost}) & (\ref{eq:def_excel_mask}) 
% & (\ref{eq:def_perf}) & (\ref{eq:def_excel_perf_cost}) & (\ref{eq:def_excel_mask}) 
% & (\ref{eq:def_perf}) & (\ref{eq:def_excel_perf_cost}) & (\ref{eq:def_excel_mask}) 
% & (\ref{eq:def_perf}) & (\ref{eq:def_excel_perf_cost}) & (\ref{eq:def_excel_mask}) 
% & (\ref{eq:def_perf}) & (\ref{eq:def_excel_perf_cost}) & (\ref{eq:def_excel_mask}) 
% & (\ref{eq:def_perf}) & (\ref{eq:def_excel_perf_cost}) & (\ref{eq:def_excel_mask}) \\
\midrule
WizardLM 13B     & 0.562 & 0 & 0 & 0.796 & 0 & 0 & 0.363 & 0 & 0 & 0.600 & 0 & 0 & 0.510 & 0 & 0 & 0.492 & 0 & 0 & 0.657 & 0 & 0 \\
Mistral 7B       & 0.558 & 0 & 0 & 0.779 & 0 & 0 & 0.349 & 0 & 0 & 0.517 & 0 & 0 & 0.561 & 0 & 0 & 0.399 & 0 & 0 & 0.640 & 0 & 0 \\
Mixtral 8x7B     & 0.721 & 0.721 & 1 & 0.920 & 0.920 & 1 & 0.572 & 0.572 & 1 & 0.634 & 0 & 0 & 0.673 & 0.673 & 1 & 0.485 & 0 & 0 & 0.837 & 0.837 & 1 \\
Code Llama 34B   & 0.553 & 0 & 0 & 0.795 & 0 & 0 & 0.464 & 0 & 0 & 0.431 & 0 & 0 & 0.612 & 0 & 0 & 0.424 & 0 & 0 & 0.635 & 0 & 0 \\
Yi 34B           & 0.727 & 0.727 & 1 & 0.937 & 0.937 & 1 & 0.331 & 0 & 0 & 0.834 & 0.834 & 1 & 0.743 & 0.743 & 1 & 0.509 & 0.509 & 1 & 0.873 & 0.873 & 1 \\
GPT-3.5          & 0.700 & 0.700 & 1 & 0.907 & 0.907 & 1 & 0.649 & 0.649 & 1 & 0.695 & 0.695 & 1 & 0.623 & 0.623 & 1 & 0.543 & 0.543 & 1 & 0.844 & 0.844 & 1 \\
Claude Instant V1& 0.368 & 0 & 0 & 0.862 & 0 & 0 & 0.547 & 0 & 0 & 0.704 & 0.704 & 1 & 0.507 & 0 & 0 & 0.561 & 0.561 & 1 & 0.812 & 0 & 0 \\
Llama 70B        & 0.629 & 0 & 0 & 0.853 & 0 & 0 & 0.300 & 0 & 0 & 0.627 & 0 & 0 & 0.498 & 0 & 0 & 0.486 & 0 & 0 & 0.784 & 0 & 0 \\
Claude V1        & 0.312 & 0 & 0 & 0.920 & 0.920 & 1 & 0.497 & 0 & 0 & -0.131 & 0 & 0 & 0.516 & 0 & 0 & 0.099 & 0 & 0 & 0.798 & 0 & 0 \\
Claude V2        & 0.456 & 0 & 0 & 0.840 & 0 & 0 & 0.567 & 0.567 & 1 & -0.554 & 0 & 0 & 0.392 & 0 & 0 & -0.011 & 0 & 0 & 0.454 & 0 & 0 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

We then use the metadata in Table~\ref{table:Table_1_routerb} and the induced Table~\ref{table:weighting} to calculate the scores $s_k$.
The most straightforward way is to take only the performance columns in Table~\ref{table:Table_1_routerb}, which we call \texttt{Perf}.
For instance, taking the performance values in the fifth row of Table~\ref{table:Table_1_routerb}, we obtain $s_{\textrm{Yi 34B}}^{(\texttt{Perf})} = (0.743, 0.938, \ldots, 0.882)$.
We also implement three other scoring ways, \texttt{Perf\_cost}, \texttt{Excel\_perf\_cost}, and \texttt{Excel\_mask}. 
Using the Perf and the Cost columns in Table~\ref{table:Table_1_routerb}, scores of \texttt{Perf\_cost} is calculated by $\textrm{Perf} - \lambda \textrm{Cost}$ with $\lambda = 0.05$ being a balance parameter.
The resulting values are listed in the columns of Table~\ref{table:weighting} indexed by (i).
With \texttt{Perf\_cost} in hand, \texttt{Excel\_perf\_cost} keeps the original \texttt{Perf\_cost} score if it is ranked as the top-$\tau$ in the column and assigns $0$ otherwise. 
Here we choose $\tau=3$.
The \texttt{Excel\_perf\_cost} scores are listed under index (ii).
\texttt{Excel\_mask} further masks the nonzero values of \texttt{Excel\_perf\_cost} as $1$ and lists them under (iii) in Table~\ref{table:weighting}. 
Finally, we feed the scores $s_k$ and the model embeddings $\xi$ to (\ref{eq:def_perf}), (\ref{eq:def_excel_perf_cost}), and (\ref{eq:def_excel_mask}) to obtain the model embedding $\rho_k$.
Specifically, \texttt{Perf} and \texttt{Perf\_cost} are fed to (\ref{eq:def_perf}), \texttt{Excel\_perf\_cost} to (\ref{eq:def_excel_perf_cost}), and \texttt{Excel\_mask} to (\ref{eq:def_excel_mask}).
Using the above symbols, we can denote, for instance, the model embedding of Yi 34B calculated via text embedding model \texttt{e5b\_E4}, scoring method \texttt{Perf\_cost}, and weighting equation (\ref{eq:def_perf}) as 
$
\rho_{\textrm{Yi 34B}}^{(\texttt{e5b\_E4\_}\texttt{Perf\_cost})} = \xi^{(\texttt{e5b\_E4})} \operatorname{softmax}\left(s_{\textrm{Yi 34B}}^{(\texttt{Perf\_cost})}\right)\footnote{Note that \texttt{e5b}, \texttt{mpnet}, and \texttt{MiniLM} are text models that generate embeddings. They need to be distinguished from the LLMs, listed in the leftmost column of Table~\ref{table:weighting}, which are candidates selected to generate responses in online learning.}.
$ 
In addition, we append all $14$ metadata (Perf and Cost over seven benchmarks) of an LLM at the end of its embedding.
Let $\rho_{x}$ be the embedding of query $x$, the feature function $\phi(x, a_k)$ is computed as the normalized $\rho_{x} * \rho_{k}$. 
To compare the effectiveness of fine-tuning, we use a suffix to indicate whether a fine-tuned model or an original model generates an embedding. 
For instance, the string ``\texttt{e5b\_E4\_Excel\_perf\_cost\_exp}'' means ``belonging to the experimental group, the embedding is generated by \texttt{e5b} fine-tuned with four epochs with the \texttt{Excel\_perf\_cost} weighting mechanism'', and ``\texttt{e5b\_E4\_Excel\_perf\_cost\_ctrl}'' means ``belonging to the control group, the embedding is generated by the original \texttt{e5b} with the \texttt{Excel\_perf\_cost} weighting mechanism.

We run \texttt{OpenAItext} with one, three, and five queries, each for five runs, and average the cumulative regrets to plot three curves\footnote{Unless mentioned, each regret curve reported is the average of 5 runs.} in Figure~\ref{fig:rtb-main-a}.
\mycmt{Is it 1, 3, and 5 or one, three, and five?}
For open-sourced embdeeing models, we fine-tune to obtain \texttt{e5b\_E2}, \texttt{e5b\_E4}, \texttt{mpnet\_E2}, \texttt{mpnet\_E4}, \texttt{MiniLM\_E2}, and \texttt{MiniLM\_E4}.
For each embedding model, four weighting mechanisms (\texttt{Perf}, \texttt{Perf\_cost}, \texttt{Excel\_perf\_cost}, \texttt{Excel\_mask}) are implemented.
The corresponding control group also undergoes the online testing phase.
There are a total of 8 curves for one embedding model.
The best performed \texttt{e5b\_E4} is shown in Figure~\ref{fig:rtb-main-b}. 
Results for the other models can be found in Figure~\ref{fig:grid-rtb-models-all} from Appendix~\ref{sec:more_routerb_results}.

We obtain the following observations from the regret curves.
In Figure~\ref{fig:rtb-main-a}, the number of queries in the prompt does not affect \texttt{OpenAItext} too much.
Thus, we choose the best version, \texttt{openai\_4}, to compare with the results generated by our proposed CCFT in Figure~\ref{fig:rtb-main-b}.
First, the experimental group outperforms the control group, showing the advantage of fine-tuning.
Second, \texttt{e5b\_E4\_Excel\_perf\_cost\_exp} and \texttt{e5b\_E4\_Excel\_mask\_exp} outperform \texttt{openai\_4}, showing that even an open-sourced model, with a careful design, can generate better embeddings than a strong general-purpose model. 
Third, when examining all plots in Figure~\ref{fig:grid-rtb-models-all-b} -- \ref{fig:grid-rtb-models-all-f}, the previous two observations hold for all other embedding models, showing convincing evidence for the effectiveness of CCFT we proposed.
Fourth, by comparing \texttt{e5b\_E4\_Excel\_perf\_cost\_exp} with \texttt{e5b\_E4\_Perf\_cost\_exp}, we observe that weighting via \texttt{Excel\_perf\_cost} yields better performance than weighting via \texttt{Excel\_mask}.
\mycmt{We compare with $a^*_{t}$, not just $a^*$.}
This suggests that, instead of weighting over all categories, it is more effective to weight only the categories in which the LLM demonstrates expertise.
In addition to achieving lower accumulated regret, both \texttt{Excel\_perf\_cost} and \texttt{Excel\_mask} incorporate a performance-cost trade-off, enhancing their practical applicability and flexibility through the tunable parameter $\lambda$.
\mycmt{Compare our TS vs MixLLM's UCB approach?}

% --- 1x2 layout ---
\begin{figure}[t]
  \centering
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots/routerb_seed2_m42_set4_figure_0.pdf}
    \caption{\texttt{OpenAItext} results}
    \label{fig:rtb-main-a}
  \end{subfigure}\hfill
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots/routerb_seed1_m42_set1_figure_0.pdf}
    \caption{Fine-tuned results}
    \label{fig:rtb-main-b}
  \end{subfigure}

  \caption{RouterBench: Cumulative regret curves (lower is better).}
  \label{fig:rtb-main}
\end{figure}
% --- 1x2 layout ---








\subsubsection{Generalization to an Unseen Benchmark}

Although an online learning setting evaluates an algorithm’s adaptivity by providing sequentially and randomly shuffled inputs, the algorithm may still access metadata from all benchmarks during the offline stage.
To more rigorously assess adaptivity to an unseen benchmark, we modify the data-generation pipeline to ensure that one benchmark remains completely hidden from the algorithm throughout both the offline and online phases.
The queries and metadata of MT-Bench are removed, as its dataset is not large enough to induce a distribution shift scenario in the coming experiment.
For the remaining six benchmarks, the metadata for ARC is removed from Table~\ref{table:Table_1_routerb}, ensuring that the algorithm is oblivious to it from the outset.
An online learning sequence is composed of two sections.
First, we sample 60 queries from each benchmark, excluding ARC (i.e., five benchmarks in total), resulting in 300 queries. 
These are randomly shuffled to form the first section of the sequence.
Next, for the second section, we sample 120 queries from ARC and an additional 300 non-overlapping queries from the other five benchmarks, following the same procedure as in the first section. These 420 (i.e., $120 + 300$) queries are then shuffled to form the second section of the learning sequence.
This setup introduces a shift in the query distribution during the second section of online learning, as queries from a previously unseen benchmark are added to evaluate the robust generalization capability of the proposed method.
Due to the modification in how metadata is accessed, we introduce an additional suffix, \texttt{ideal}, which allows the model to access ARC's metadata.
Although the \texttt{ideal} case is not realistic in practice, comparing results from configurations ending with \texttt{ideal} and those ending with \texttt{exp} enables us to assess the adaptivity strength of our method.
For the rest of the experimental setting, we follow the same fine-tuning protocol in the last section to generate embeddings.
Based on the observations from Figures~\ref{fig:rtb-main-b} and~\ref{fig:grid-rtb-models-all}, we implement the \texttt{Excel\_perf\_cost} and \texttt{Excel\_mask} weighting schemes due to their consistently strong performance.

The results of \texttt{OpenAItext} and \texttt{e5b} are shown in Figure~\ref{fig:rbst-main}.
Results for \texttt{mpnet} and \texttt{MiniLM} can be found in Figure~\ref{fig:rtb-rbst-all} from Appendix~\ref{sec:more_routerb_results}.
We choose \texttt{openai\_0} to compare with the results generated by \texttt{e5b\_E4} according to Figure~\ref{fig:rbst-main-a}.
First, obviously, the fine-tuning group outperforms the control group.
Second, \texttt{e5b\_E4\_Excel\_perf\_cost\_exp} and \texttt{e5b\_E4\_Excel\_mask\_exp}, the fine-tuning results via our CCFT method outperform that of \texttt{openai\_0}.
The case in the second observation holds for Figure~\ref{fig:rtb-rbst-all-a} through Figure~\ref{fig:rtb-rbst-all-e}, justifying the effectiveness of the proposed method.
\mycmt{However, due to the unseen benchmark, the curve gaps between \texttt{openai\_0} become closer (REALLY?) to that in Figure~\ref{fig:rtb-main-b}. I need to plot a figure to compare. Maybe openai\_0 suffers more in unseen benchmark.} 
Third, interestingly, we find that it is not always the case that an \texttt{ideal} curve outperforms the corresponding \texttt{exp} curve.
One can find this by comparing pair (\texttt{e5b\_E4\_Excel\_perf\_cost\_exp}, \texttt{e5b\_E4\_Excel\_perf\_cost\_ideal}) with pair (\texttt{e5b\_E4\_Excel\_mask\_exp}, \texttt{e5b\_E4\_Excel\_mask\_ideal}).
The situation also can be found in Figure~\ref{fig:rtb-rbst-all}.
\mycmt{In particular, in Figure~\ref{fig:rtb-rbst-all-d} and \ref{fig:rtb-rbst-all-e}.}
This phenomenon suggests weighting less may be better than weighting more, and it may be related to the last observation we have in the original RouterBench experiments that weighting over all benchmark embeddings is not a good idea.
Maybe the metadata alone is not enough for us to make a weighting judgment; we might need to look into other aspects of the benchmarks in future work.



\begin{figure}[t]
  \centering
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots/routerb_rbst2_m42_set4_figure_0.pdf}
    \caption{OpenAI variants}
    \label{fig:rbst-main-a}
  \end{subfigure}\hfill
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots/routerb_rbst1_m42_set1_figure_0.pdf}
    \caption{E5b variants}
    \label{fig:rbst-main-b}
  \end{subfigure}

  \caption{Robust generalization: Cumulative regret curves (lower is better).}
  \label{fig:rbst-main}
\end{figure}








\subsection{MixInstruct}
\label{sec:exp_mixInst}
MixInstruct \citep{jiang2023mixinst_blender} is a 110K-example instruction-following benchmark built to evaluate LLM routing methods. 
It mixes data from four sources (Alpaca-GPT4, Dolly-15K, GPT4All-LAION, ShareGPT) with a 100k/5k/5k train/dev/test split. 
The authors run eleven popular open-source LLMs on the full set, then derive oracle pairwise preferences by prompting ChatGPT to compare every candidate pair per example.

\begin{table}[h!]
\caption{Models Ranked First by Percentage of Examples}
\label{table:mix-inst-top-percentage}
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lccccccccccc}
\toprule
\textbf{Model} & Vicuna & MOSS & Open Assistant & Alpaca & Baize & ChatGLM & MPT & Koala & Dolly V2 & StableLM & FLAN-T5 \\
\midrule
\textbf{Percentage (\%)} & 21.22 & 12.91 & 12.61 & 11.61 & 11.61 & 8.51 & 7.61 & 6.71 & 4.50 & 1.90 & 0.80 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
% \mycmt{MixInstruct table is generated by \url{https://chatgpt.com/c/68cc1655-c370-8322-8021-c70b7cb8ea78}.}

Table~\ref{table:mix-inst-top-percentage}, adapted from Figure 1 of \cite{jiang2023mixinst_blender}, underscores the importance of LLM routing: selecting the best-matching LLM for each query is crucial, as any fixed-LLM strategy will yield no more than 22\% accuracy.
A distinctive characteristic of the MixInstruct dataset is the absence of an explicit category label, rendering the proposed methods in (\ref{eq:def_perf}), (\ref{eq:def_excel_perf_cost}), and (\ref{eq:def_excel_mask}) infeasible.
Since this challenge can naturally arise in practical settings, we use MixInstruct to evaluate our alternative formulation presented in (\ref{eq:def_mix_inst}), thereby validating its applicability under realistic constraints.
Moreover, the pairwise comparison labels in MixInstruct make it closely resemble datasets commonly encountered in industrial applications.

To make the regret defined in (\ref{eq:regret}) computable, we reconstruct the utility function $r^{*}(x, a)$.
Pairwise comparisons between LLM candidates are translated into scores by adding a win value of 1, a tie 0.5, and a loss 0.
During the translation process, a Condorcet winner may emerge \citep{black1958,wiki_condorcet_winner}. 
To ensure it receives the highest score, we assign the Condorcet winner a top score with an additional bonus.
During the data analysis stage, we found the existence of ambiguous queries. 
We apply the OpenAI API to assign an ambiguity score to each query and remove the most ambiguous 8\% and 15\% of queries.
The ambiguity removal process introduces additional sub-strings \texttt{\_8} and \texttt{\_15} in the naming of regret curves. 
Using (\ref{eq:def_mix_inst}), the rest of the experiment setup follows the procedure described in Section~\ref{sec:exp_routerb}.
We obtain Figure~\ref{fig:mixinst-main} and deferred Figure~\ref{fig:mixinst-15} to Appendix~\ref{sec:more_mixinst} due to space limit.

\begin{figure}[h]
  \centering
  % Left plot
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots/mixinst_seed_m1_set1_figure_0.pdf}
    \caption{Implementations of (\ref{eq:def_mix_inst}) versus \texttt{openai} variants}
    \label{fig:mixinst-main-8}
  \end{subfigure}\hfill
  % Right plot
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots/mixinst_seed_m1_set2_figure_0.pdf}
    \caption{Comparing ambiguity removal: 8\% versus 15\%}
    \label{fig:mixinst-main-compare}
  \end{subfigure}

  \caption{MixInstruct: Cumulative regret curves (lower is better).}
  \label{fig:mixinst-main}
\end{figure}

In Figure~\ref{fig:mixinst-main-8}, we again observe that implementations of the proposed (\ref{eq:def_mix_inst}) outperform \texttt{openai} variants, demonstrating that our approach remains effective even when the dataset lacks metadata information.
When comparing results under different degrees of ambiguity removal, we observe a consistent pattern in Figure~\ref{fig:mixinst-main-compare} across \texttt{e5b\_E4}, \texttt{mpnet\_E4}, and \texttt{openai\_4}: removing the top 15\% of ambiguous queries is worse than removing only the top 8\%. 
This highlights the risk of discarding learnable information when too many queries are removed.




\section{Concluding Remarks and Future Work}

(1) Integrate the preference feedback and rating scale feedback.
Our method considers dueling feedback currently. 
It can be easily modified to take rating scale feedback.
However, a challenge is to integrate both. 
It is unclear how to build an online learner that takes both forms of input.

(2) Dynamically retrain the model embedding.
The proposed model embedding is trained by a fixed offline dataset.
As time goes on, the service provider will receive new annotated information.
It would be interesting to construct a mechanism that adapts the model embedding to reflect the newly available dataset.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection*{Author Contributions}
% Optional.

% \subsubsection*{Acknowledgments}
% \mycmt{All acknowledgments, including those to funding agencies, go at the end of the paper.}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibliography{iclr2026/bibtex_llm-routing}
\bibliographystyle{iclr2026_conference}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage

\appendix


\section{MMLU Supplementary Materials}
\label{sec:more_mmlu}


\begin{figure*}[h]
  \centering
  \includegraphics[width=0.95\linewidth]{plots/tsne_3d_side_by_side.pdf}
  \caption{3D t-SNE visualization of experimental (left) and control (right) groups. Each point represents an embedding projected into 3D space, with colors indicating cluster membership.}
  \label{fig:tsne-3d}
\end{figure*}
\mycmt{t-SNE and 3D t-SNE plots?}



\section{RouterBench Supplementary Materials}
\label{sec:more_routerb}


\subsection{Categorical Weighting}
\label{sec:more_categorical_weighting}

\begin{table}[htbp]
\centering
\caption{Performance and cost across benchmarks}
\label{table:Table_1_routerb}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccccccccccccc}
\toprule
\textbf{LLM} & 
\multicolumn{2}{c}{\textbf{MMLU}} & 
\multicolumn{2}{c}{\textbf{MT-Bench}} & 
\multicolumn{2}{c}{\textbf{MBPP}} & 
\multicolumn{2}{c}{\textbf{HellaSwag}} & 
\multicolumn{2}{c}{\textbf{Winogrande}} & 
\multicolumn{2}{c}{\textbf{GSM8k}} & 
\multicolumn{2}{c}{\textbf{ARC}} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
\cmidrule(lr){8-9}
\cmidrule(lr){10-11}
\cmidrule(lr){12-13}
\cmidrule(lr){14-15}
& Perf$\uparrow$ & Cost$\downarrow$ 
& Perf$\uparrow$ & Cost$\downarrow$ 
& Perf$\uparrow$ & Cost$\downarrow$ 
& Perf$\uparrow$ & Cost$\downarrow$ 
& Perf$\uparrow$ & Cost$\downarrow$ 
& Perf$\uparrow$ & Cost$\downarrow$ 
& Perf$\uparrow$ & Cost$\downarrow$ \\
\midrule
WizardLM 13B     & 0.568 & 0.122 & 0.796 & 0.006 & 0.364 & 0.011 & 0.636 & 0.727 & 0.512 & 0.040 & 0.510 & 0.354 & 0.660 & 0.068 \\
Mistral 7B       & 0.562 & 0.081 & 0.779 & 0.003 & 0.349 & 0.006 & 0.541 & 0.485 & 0.562 & 0.027 & 0.409 & 0.210 & 0.642 & 0.046 \\
Mixtral 8x7B     & 0.733 & 0.245 & 0.921 & 0.012 & 0.573 & 0.023 & 0.707 & 1.455 & 0.677 & 0.081 & 0.515 & 0.594 & 0.844 & 0.137 \\
Code Llama 34B   & 0.569 & 0.317 & 0.796 & 0.015 & 0.465 & 0.021 & 0.525 & 1.882 & 0.617 & 0.104 & 0.462 & 0.752 & 0.644 & 0.177 \\
Yi 34B           & 0.743 & 0.326 & 0.938 & 0.018 & 0.333 & 0.031 & 0.931 & 1.938 & 0.748 & 0.107 & 0.552 & 0.867 & 0.882 & 0.182 \\
GPT-3.5          & 0.720 & 0.408 & 0.908 & 0.026 & 0.651 & 0.044 & 0.816 & 2.426 & 0.630 & 0.134 & 0.601 & 1.170 & 0.855 & 0.228 \\
Claude Instant V1& 0.384 & 0.327 & 0.863 & 0.030 & 0.550 & 0.064 & 0.801 & 1.943 & 0.512 & 0.108 & 0.626 & 1.300 & 0.821 & 0.183 \\
Llama 70B        & 0.647 & 0.367 & 0.854 & 0.022 & 0.302 & 0.039 & 0.736 & 2.183 & 0.504 & 0.121 & 0.529 & 0.870 & 0.794 & 0.205 \\
Claude V1        & 0.475 & 3.269 & 0.938 & 0.361 & 0.527 & 0.607 & 0.841 & 19.43 & 0.570 & 1.077 & 0.653 & 11.09 & 0.889 & 1.829 \\
Claude V2        & 0.619 & 3.270 & 0.854 & 0.277 & 0.605 & 0.770 & 0.421 & 19.50 & 0.446 & 1.081 & 0.664 & 13.49 & 0.546 & 1.833 \\
GPT-4            & 0.828 & 4.086 & 0.971 & 0.721 & 0.682 & 1.235 & 0.923 & 24.29 & 0.858 & 1.346 & 0.654 & 19.08 & 0.921 & 2.286 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

Tables \ref{table:Table_1_routerb} and \ref{table:weighting} are from \url{https://chatgpt.com/c/68cb776a-3fbc-8329-b5a1-3cf59d40b1f5}


% \begin{table}[h!]
% \label{table:hypothetic_method}
% \centering
% \caption{LLM Scores Across Categories}
% \begin{tabular}{lccccccc}
% \toprule
%  & Category 1 & Category 2 & Category 3 & Category 4 & Category 5 & Category 6 & Category 7 \\
%   & $\xi_1$ & $\xi_2$ & $\xi_3$ & $\xi_4$ & $\xi_5$ & $\xi_6$ & $\xi_7$ \\
% \midrule
% LLM $a_1$ & 0.368 & 0.862 & 0.547 & \textbf{0.704} & 0.507 & \textbf{0.561} & 0.812 \\
% LLM $a_2$ & 0.629 & 0.853 & 0.300 & 0.627 & 0.498 & 0.486 & 0.784 \\
% LLM $a_3$ & \textbf{0.721} & \textbf{0.920} & \textbf{0.572} & 0.634 & \textbf{0.673} & 0.485 & \textbf{0.837} \\
% LLM $a_4$ & \textbf{0.727} & \textbf{0.937} & 0.331 & \textbf{0.834} & \textbf{0.743} & \textbf{0.509} & \textbf{0.873} \\
% LLM $a_5$ & 0.456 & 0.840 & \textbf{0.567} & -0.554 & 0.392 & -0.011 & 0.454 \\
% \bottomrule
% \end{tabular}
% \end{table}

% Using the hypothetical table above, we present 
% \bcmt{(maybe move to appendix or delete).}





\subsection{Additional Results}
\label{sec:more_routerb_results}

Figure~\ref{fig:grid-rtb-models-all} lists the cumulative regret curves for \texttt{e5b\_E2}, \texttt{mpnet\_E4}, \texttt{mpnet\_E2}, \texttt{MiniLM\_E4}, and \texttt{MiniLM\_E2}.
Figure~\ref{fig:grid-rtb-models-all-a} compares all embedding models with \texttt{Excel\_perf\_cost} and \texttt{Excel\_mask} mechanisms, which are the better weighting method most of the time.

% --- 3-by-2 Figure ---
\begin{figure*}[h]
  \centering
  % Row 1
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots/routerb_seed1_m42_set2_figure_0.pdf}
    \caption{Compare against text models.}
    \label{fig:grid-rtb-models-all-a}
  \end{subfigure}\hfill
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots/routerb_seed1_m42_set1_figure_1.pdf}
    \caption{\texttt{e5b\_E2} results.}
    \label{fig:grid-rtb-models-all-b}
  \end{subfigure}

  \vspace{0.3em}

  % Row 2
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots/routerb_seed1_m42_set1_figure_2.pdf}
    \caption{\texttt{mpnet\_E4} results.}
  \end{subfigure}\hfill
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots/routerb_seed1_m42_set1_figure_3.pdf}
    \caption{\texttt{mpnet\_E2} results.}
  \end{subfigure}

  \vspace{0.3em}

  % Row 3
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots/routerb_seed1_m42_set1_figure_4.pdf}
    \caption{\texttt{MiniLM\_E4} results.}
  \end{subfigure}\hfill
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots/routerb_seed1_m42_set1_figure_5.pdf}
    \caption{\texttt{MiniLM\_E2} results.}
    \label{fig:grid-rtb-models-all-f}
  \end{subfigure}

  \caption{RouterBench: Cumulative regret curves (lower is better).}
  \label{fig:grid-rtb-models-all}
\end{figure*}
% --- 3-by-2 Figure ---


% % --- 2-by-3 Figure ---
% \begin{figure*}[t]
%   \centering
%   \begin{subfigure}{0.32\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{plots/routerb_seed1_m42_set1_figure_0.pdf}
%     \caption{A}
%   \end{subfigure}\hfill
%   \begin{subfigure}{0.32\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{plots/routerb_seed1_m42_set1_figure_1.pdf}
%     \caption{B}
%   \end{subfigure}\hfill
%   \begin{subfigure}{0.32\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{plots/routerb_seed1_m42_set1_figure_2.pdf}
%     \caption{C}
%   \end{subfigure}

%   \vspace{0.3em}

%   \begin{subfigure}{0.32\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{plots/routerb_seed1_m42_set1_figure_3.pdf}
%     \caption{D}
%   \end{subfigure}\hfill
%   \begin{subfigure}{0.32\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{plots/routerb_seed1_m42_set1_figure_4.pdf}
%     \caption{E}
%   \end{subfigure}\hfill
%   \begin{subfigure}{0.32\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{plots/routerb_seed1_m42_set1_figure_5.pdf}
%     \caption{F}
%   \end{subfigure}

%   \caption{Cumulative regret curves.}
%   \label{fig:grid-rtb-models}
% \end{figure*}
% % --- 2-by-3 Figure ---


\begin{figure*}[h]
  \centering
  % Row 1
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots/routerb_rbst1_m42_set1_figure_1.pdf}
    \caption{A}
    \label{fig:rtb-rbst-all-a}
  \end{subfigure}\hfill
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots/routerb_rbst1_m42_set1_figure_2.pdf}
    \caption{B}
    \label{fig:rtb-rbst-all-b}
  \end{subfigure}

  \vspace{0.3em}

  % Row 2
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots/routerb_rbst1_m42_set1_figure_3.pdf}
    \caption{C}
    \label{fig:rtb-rbst-all-c}
  \end{subfigure}\hfill
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots/routerb_rbst1_m42_set1_figure_4.pdf}
    \caption{D}
    \label{fig:rtb-rbst-all-d}
  \end{subfigure}

  \vspace{0.3em}

  % Row 3
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots/routerb_rbst1_m42_set1_figure_5.pdf}
    \caption{E}
    \label{fig:rtb-rbst-all-e}
  \end{subfigure}\hfill
  % \begin{subfigure}{0.45\textwidth}
  %   \centering
  %   \includegraphics[width=\linewidth]{plots/routerb_rbst1_m42_set1_figure_0.pdf}
  %   \caption{F}
  %   \label{fig:rbst3x2-f}
  % \end{subfigure}

  \caption{Robust generalization: Cumulative regret curves (lower is better).}
  \label{fig:rtb-rbst-all}
\end{figure*}

\mycmt{Figure comes from \url{https://chatgpt.com/c/68cbf7d5-e4fc-832d-a9a0-5c5c1f1c193a}.}





\section{MixInstruct Supplementary Materials}
\label{sec:more_mixinst}



\subsection{Additional Results}
\label{sec:more_mixinst_results}

\mycmt{Add Figure~\ref{fig:mixinst-fig1}.}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\linewidth]{plots/mixinst_seed_m1_set1_figure_1.pdf}
  \caption{MinInstruct: Cumulative regret curves (lower is better).}
  \label{fig:mixinst-15}
\end{figure}






==> iclr2026/96_main_ver1_250921.tex <==




\section{Introduction}
\label{sec:intro}
The potential of LLMs is so large that it almost becomes a necessary part of daily life, with applications from office assistance, fashion/dining suggestions, to entertainment.
LLM routing refers to a problem of dynamically selecting the most suitable LLM from a set of candidates for each query from a sequence of questions.
Before the emergence of a universally dominant and affordable foundation model, routing is important as a suitable LLM matches the user traits, the model expertise, and the cost.
To balance these three key factors, cascading algorithms FrugalGPT \citep{chen2024frugalgpt} and AutoMix \citep{AggarwalMAPMZGR24} were first proposed.
The idea is to query a cheap model first and advance the query to a more expensive model if the current reply is likely to fail the user’s expectation.

A drawback of cascading is the accumulated cost and latency caused by a series of calls to multiple LLM candidates to obtain the final reply to output.
To avoid this, supervised routing methods \citep{shnitzer2023llmrouting, lu2024zooter, ding2024hybridllm, hu2024routerbench, srivatsa2024harnessing} were proposed.
In general, a supervised router reduces the latency by applying a classification or a regression prediction before the LLM query.
The supervised approach has evolved into branches. 
A branch studied ensembles \citep{jiang2023mixinst_blender, maurya-etal-2025-selectllm, zhang2025avengers, zhang2025avengerspro}, which allows the agent to select a subset or fuse answers. 
Another branch exercised cost-aware model assignment \citep{sakota2024forc, hu2024routerbench, liu2024optllm} to balance the cost and performance.
There are also works that combine representation learning \citep{feng2025graphrouter, zhuang2025embedllm} to strengthen the user and model’s semantic information before training.

For supervised routing methods, having abundant real-valued annotations with high-quality label information is critical for successful classification or regression training.
Unfortunately, such a requirement is often unrealistic in the context of LLM routing.
In some cases, users are either reluctant or unmotivated to provide feedback. 
They may also be unable to quantify their satisfaction, especially when dealing with open-ended questions or when they lack the ability to verify the correctness of the LLM's response.
To ease the annotation burden, some efforts focused on weak supervision \citep{sugiyama2022weak, chiang2025unified}, which only collect binary feedback such as like/dislike or pairwise comparison \citep{ong2025routellm, zhao2024eagle, wang2025mixllm}.
The advantage is that one-click feedback is user-friendly, and it is more confident to say reply A is better than B than to assign reply A a score out of ten.
The reason that makes a weakly supervised approach appealing is that, as shown by the referred papers, the binary feedback can be translated into a model ranking or an estimate of the labeling function. 

In addition to the challenge of annotation, adaptivity remains a key challenge to be addressed in developing a usable routing system.
Shifts in query distributions, such as changes in trending topics like fashion or temporal variations between work hours and leisure time, introduce non-stationary conditions. 
Moreover, new LLMs and benchmarks are continuously introduced, resulting in a constantly evolving environment for routing.
These evolving conditions often exceed the capacity of static, supervised learning-based routing policies. 
Addressing such challenges in a dynamic environment is a key motivation for adopting online learning approaches for LLM routing, as they offer the ability to continuously learn and optimize the routing policy in real time.
The online algorithms adopted in prior work can be categorized into three classes: multi-armed bandits \citep{nguyen2024metallm, dai2024C2MAB-V, li2025llmbandit}, contextual bandits \citep{wang2025mixllm}, and reinforcement learning \citep{sikeridis2025pickllm}.

To build a practical routing system to fit the various requests, multiple challenges should be addressed simultaneously. 
However, we notice that there was little effort at jointly solving the challenges of adaptivity and weak supervision, even if the community has already made huge progress in respective directions.
To our best knowledge, \cite{wang2025mixllm} is the only attempt to address adaptivity and pointwise feedback (e.g., like/dislike) at the same time.
Therefore, this paper focuses on investigating LLM routing under a stochastic bandit setting, which captures the dynamics of a changing environment, and operates under weak supervision in the form of pairwise preference feedback (e.g., reply A is preferred over reply B)\footnote{\bcmt{[CK] Let's fix a term. Reply or response?}}.
The advantages of the project are threefold:
First, we introduce the contextual dueling bandit algorithm FGTS.CDB \citep{li2024fgtscdb} as the core module.
It naturally combines weak supervision (i.e., the dueling feedback) and adaptive learning (i.e., the bandit algorithm) in the algorithm input and the design of the learning procedure.
Its introduction provides the community with broader methodological choices for future research.
Second, it is a theoretically justified method that offers a clear explanation of how binary feedback is connected to the utility function that defines the model's performance, which is a complex function of user satisfaction, model expertise, and model cost.
Third, it provides a platform for us to investigate what makes it work and what makes it fail, so that we can realize it to be the first\mycmt{(?)} practical LLM router that does not require high-quality annotations and is robust to dynamically changing environments.

The paper’s contributions are summarized as follows.
\begin{itemize}
    \item We propose Category-Calibrated Fine-Tuning (CCFT), a generic embedding method to encode an LLM’s expertise.
    The feature function constructed by CCFT allows us to build the first trainable contextual dueling learner in LLM routing.
    \item Strong evidence of the efficacy of the proposed method is observed from experimenting with two real-world datasets, RouterBench \citep{hu2024routerbench} and MixInstruct \citep{jiang2023mixinst_blender}.
    All four implementations of CCFT are tested and compared to each other.
    The curves of cumulative regret demonstrate the behavior of the proposed method converging to the optimal strategy that chooses the best matching model for each question.
    \item The proposed methods also demonstrate the merits of robust generalization to an unseen benchmark and performance-cost balance.
    \item In the experiments, several common practices of LLM, including prompting, context fine-tuning, open-sourced and block-box text embedding models, are integrated with the proposed method, accumulating substantial knowledge and skills of addressing LLM routing.
\end{itemize}




\section{Related Work}

\subsection{LLM Routing}
\label{sec:related_routing}
\citet{ong2025routellm}

\subsection{Contextual Dueling Bandits and Feel-Good Thompson Sampling}
\label{sec:bandits}
Research on contextual dueling bandits has advanced along several directions. \cite{kumagai2017continuousdueling} analyzed dueling bandits with a continuous action space and, under strong convexity and smoothness, established dimension-free regret guarantees. Building on preference models, \cite{bengs2022stochasticcontextual} introduced the CoLSTIM algorithm for stochastic contextual dueling bandits under linear stochastic transitivity, providing learning guarantees tailored to this structure. Recently, \cite{di2024varianceaware} proposed VACDB, an action-elimination-based method that achieves tighter, variance-dependent regret bounds for contextual settings.

Feel-Good Thompson Sampling (FGTS) was proposed to reconcile Thompson sampling’s strong empirical performance with frequentist-style guarantees \citep{zhang2022fgts}. \cite{fan2023powerfgts} offered a unified analysis framework showing how FGTS yields robust guarantees across several linear contextual bandit variants. The FGTS idea has also been extended to reinforcement learning, e.g., Model-based Optimistic Posterior Sampling (MOPS) for Markov decision processes \citep{agarwal2022modelbasedops}. To our best knowledge, our work is the first to apply FGTS to LLM routing, connecting preference-based bandit principles with practical model-selection pipelines.


\section{Background}
\label{sec:background}

\subsection{Feel-Good Thompson Sampling for Contextual Dueling Bandits}
\rcmt{Need a section level symbol refinement.}
The contextual dueling bandit problem can be seen as a repeated game between a bandit algorithm and an environment for T rounds. 
In each round $t = 1, 2, \ldots T$, the algorithm observes a contextual vector $x_t$ from the environment.
% In each round $t = 1, 2, \ldots T$, the algorithm observe a contextual vector $x_t$ representing the query from the environment.
Then, the algorithm selects two actions $a^1_t, a^2_t \in \mathcal{A} = \{k\}_{k=1}^{K}$\mycmt{(resp. $\{a_k\}_{k=1}^{K}$)} as responses.
After presenting the responses, the algorithm observes a preference feedback $y_t$.
The performance of the algorithm is measured by its cumulative regret 
\eqary{
    \operatorname{Regret}(T) 
    := \sum_{t=1}^{T} \left[ r^{*}(x_t, a_t^{*}) - \frac{r^{*}(x_t, a_t^{1}) + r^{*}(x_t, a_t^{2})}{2} \right],
    \num\label{eq:regret}
}
where $r^{*}(x, a)$ is the utility function and $a_t^{*} = \arg\max_{a \in \mathcal{A}} r^{*}(x_t, a)$ is the best action for input $x_t$.

The setting fits seamlessly to the LLM routing problem studied in this paper if we view $x_t$ as the query embedding,
% that encodes query semantics and user traits, 
$a^1_t$ and $a^2_t$ as two LLMs, $y_t$ as the preference feedback, and the $r^{*}(x, a)$ as the function balancing the user satisfaction and model score\footnote{The model score is calculated from the LLM performance, cost, latency, and other interested factors.} that we want to optimize.
The connection between the weak supervision of preference feedback $y$ and the ideal supervision provided by $r^{*}(x, a)$ is captured by the Bradley--Terry--Luce (BTL) model~\citep{hunter2004btl, luce2005btl}:
Given query $x$ and two LLMs $a^1$ and $a^2$, the probability of observing $a^1$ is preferred over $a^2$ (i.e., $y=1$) is
\eqary{
    \mathbb{P}(y = 1 \mid x, a^1, a^2) 
    = 
    % \frac{\exp(r^{*}(x, a^1))}{\exp(r^{*}(x, a^1)) + \exp(r^{*}(x, a^2))}
    % = 
    \exp\big(-\sigma(r^{*}(x, a^1) - r^{*}(x, a^2))\big),
}
where $\sigma(z) = \log(1 + \exp(-z))$\footnote{
A more general setting accepting more than two candidates is called the Plackett-Luce (PL) model \citep{pmlr-v32-soufiani14, pmlr-v48-khetan16, ren2018pacranking}.
}.

\begin{algorithm}
\caption{FGTS.CDB}\label{alg:fgts-cdb}
\begin{algorithmic}[1]
\State Given action space $\mathcal{A}$ and hyperparameters $\eta, \mu$. Initialize $S_0 = \varnothing$.
\For{$t = 1, \ldots, T$}
  \State Receive query $x_t$.
  \For{$j = 1, 2$}
    \State Sample model parameter $\theta_t^{j}$ from the posterior distribution: 
    \eqary{
        p^j(\theta \mid S_{t-1}) 
        \propto 
        \exp\left( -\sum_{i=1}^{t-1} L^j(\theta, x_i, a_i^1, a_i^2, y_i) \right) p_0(\theta)
    }
    % $p^{j}(\,\cdot \mid S_{t-1})$, defined in (4.1).
    \State Select LLM $a_t^{j} = \arg\max_{a \in \mathcal{A}}\; \langle \theta_t^{j}, \,\phi(x_t,a) \rangle$ to generate the response.
  \EndFor
  \State Receive preference feedback $y_t$.
  \State Update history $S_t \leftarrow S_{t-1} \cup \{(x_t, a_t^{1}, a_t^{2}, y_t)\}$.
\EndFor
\end{algorithmic}
\end{algorithm}
Assuming the linear reward model $r^{*}(x, a) = \langle \theta^{*}, \phi(x, a) \rangle$, \cite{li2024fgtscdb} proposed Algorithm~\ref{alg:fgts-cdb} and proved that it achieves $\mathbb{E}[\operatorname{Regret}(T)] = \widetilde{\mathcal{O}}(d\sqrt{T})$, where $d$ is the dimension $\theta$. 
FGTS.CDB learns the LLM selection strategies, $\theta^{1}_t$ and $\theta^{2}_t$, in an online fashion.
Its success hinges on the posterior $p^j(\theta \mid S_{t-1})$ defined by the likelihood function
\eqary{
    L^j(\theta, x, a^1, a^2, y) 
    = 
    \eta \, \sigma\big(y \langle \theta, \phi(x, a^1) - \phi(x, a^2) \rangle \big) - \mu \max_{\tilde{a} \in \mathcal{A}} \langle \theta, \phi(x, \tilde{a}) - \phi(x, a^{3-j}) \rangle.
}
The intuition behind $L^{j}(\cdot)$ is as follows: if $\theta$ aligns well with the preference feedback $y$, that is, when $y \langle \theta, \phi(x, a^1) - \phi(x, a^2) \rangle$ is positive and large, then $\theta$ is more likely to be chosen.
The second term in the likelihood function serves as a ``feel-good'' component, encouraging the selection of a $\theta$ that outperforms past selections made by the other selection strategy\footnote{Specifically, note that, $a^{3-j} = a^2$ for $j=1$ and $a^{3-j} = a^1$ for $j=2$.}. 
As time $t$ progresses, the observation history $S_t$ accumulates, allowing FGTS to dynamically adjust its samples $\theta^{1}_{t+1}$ and $\theta^{2}_{t+1}$ accordingly.
In an evolving environment, any changes are reflected in $S_t$, and adaptivity is inherently ensured by the bandit algorithm.

Being theoretically oriented, \cite{li2024fgtscdb} assumes that the feature function $\phi(x, a)$ is given and perfect. 
However, this assumption generally does not hold in real-world applications.
In Section~\ref{sec:failure_cases}, we demonstrate how an imperfect $\phi(x, a)$ can hinder learning and highlight a key obstacle in applying FGTS.CDB to the routing problem.
Subsequently, in Section~\ref{sec:proposed_model_emb}, we introduce our method for constructing a feature function that enables FGTS.CDB, with the aforementioned merits, to function effectively in practical LLM routing scenarios.


% \subsection{Context Contrastive Fine-Tuning}
% \rcmt{Here or Appendix?}


% \subsection{Materials}

% \noindent\textbf{Stochastic Preference Model.} 
% In this work, we assume that the preference $y_t$ follows a Bernoulli distribution 
% according to the Bradley--Terry--Luce (BTL) model~\cite{Hunter2004,Luce2005}: 
% Given context $x_t$ and responses $a_t^1, a_t^2$, 
% the probability of $a_t^1$ being preferred over $a_t^2$ is
% \eqary{
%     \mathbb{P}(y_t = 1 \mid x_t, a_t^1, a_t^2) 
%     = 
%     \frac{\exp(r^{*}(x_t, a_t^1))}{\exp(r^{*}(x_t, a_t^1)) + \exp(r^{*}(x_t, a_t^2))}
%     = 
%     \exp\big(-\sigma(r^{*}(x_t, a_t^1) - r^{*}(x_t, a_t^2))\big),
% }
% where $\sigma(z) = \log(1 + \exp(-z))$\footnote{
% A more general setting accepting more than two candidates is called the Plackett-Luce (PL) model \cite{Soufiani et al., 2014; Khetan & Oh, 2016; Ren et al., 2018}.
% }.

% \noindent\textbf{Learning Objective.} 
% The goal is to minimize the cumulative average regret:
% \eqary{
%     \operatorname{Regret}(T) 
%     := \sum_{t=1}^{T} \left[ r^{*}(x_t, a_t^{*}) - \frac{r^{*}(x_t, a_t^{1}) + r^{*}(x_t, a_t^{2})}{2} \right],
% }
% where $a_t^{*} = \arg\max_{a \in \mathcal{A}} r^{*}(x_t, a)$ is the optimal LLM for question $x_t$.




\section{A Generic Representation Learning Method}
\label{sec:generic_method}

\subsection{The Failure of Naive Implementations}
\label{sec:failure_cases}
This subsection demonstrates the practical challenge of a carefully designed feature function.
We chose five topics\footnote{They are abstract algebra, anatomy, astronomy, international law, and machine learning.} from MMLU. 
Questions are sampled to form the offline learning and online testing sets.
We assume there are five LLMs, each with expertise in one of the topics.
We tried two ways to generate the model embeddings $\rho_k$.
\mycmt{(revise?) We use $a_k$ to both index an LLM and denote its model embedding; this would simplify the symbols.}
\rcmt{(revise?) Replace $\rho_k$ with $a_k$.}
Each way takes the offline questions of one topic and is repeated\mycmt{(?)} five times to build five model embeddings.
In the first way, we encode the model description via OpenAI's \texttt{text-embedding-3-large}, where the model description is the combination of our handcrafted prompt with offline questions.
In the second way, we first generate offline question embeddings using \texttt{text-embedding-3-large} and then take their average as the model embedding of the corresponding topic. 
The intuition behind both approaches is to represent a model using the sample questions it excels at.
It is rather simple to generate a question embedding $x$, as we simply feed the question string into \texttt{text-embedding-3-large}.
We tested the Hadamard product (element-wise multiplication) $\phi(x, a) = x * a$\mycmt{(integrate with $\rho_k$? Or simply use text to refer $a_k$ as both index and embedding?)} with normalization and vector addition (element-wise addition) $\phi(x, a) = x + a$ with normalization to construct $\phi$ and keep the first one based on the experimental outcomes.

\begin{figure}[htbp]
    \centering
    
    % Subfigure (a)
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\linewidth]{fgts_regret_fgts-llm-mmlu_001+.png}
        \caption{FGTS.CDB with the first model embedding method}
        \label{fig:a}
    \end{subfigure}
    \hfill
    % Subfigure (b)
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\linewidth]{fgts_regret_fgts-llm-mmlu_250406_006+.png}
        \caption{FGTS.CDB with the second model embedding method}
        \label{fig:b}
    \end{subfigure}
    \hfill
    % Subfigure (c)
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\linewidth]{0711_m1_off10_sample200_mq400_openai_0_vs_e5b_E4_exp+.png}
        \caption{A successful example of the blue curve}
        \label{fig:c}
    \end{subfigure}

    \caption{Failure vs Success Learning in Contextual Dueling Bandits (FGTS.CDB). Cumulative regret is shown across evaluation rounds. A flat slope indicates good learning progress, as it reflects a slow accumulation of regret.}
    \label{fig:failure_exs}
\end{figure}
% \bcmt{(Figure creation: \url{https://chatgpt.com/c/68be7116-5bb0-8324-bdea-ab37025f7b70})}
From Figure\ref{fig:failure_exs} (a) and (b), we see that the slope almost does not change with rounds. 
This means the regret keeps accumulating, and hence the learning does not progress a lot.
In contrast, the slope of the blue curve in Figure\ref{fig:failure_exs} (c) reduces as the rounds increase. 
This small cumulative regret reflects that the learning agent is making fewer and fewer mispredictions and converging the behavior toward the best routing strategy. 
In the next subsection, we propose a generic method to construct model embeddings achieving a similar behavior to Figure\ref{fig:failure_exs} (c) and then test its realizations on real-world datasets in experiments.



\subsection{The Proposed Method}
\label{sec:proposed_model_emb}

Note that by design, $\phi(x_t, a)$ combines the information from the user side, $x_t$, and the information from the LLM side, $a$.
Since the text models we selected are well-recognized sentence encoders, the failure cases discussed in Section~\ref{sec:failure_cases} are most likely due to careless design of the model embeddings.
% Therefore, it is imperative to ensure that $a_k$ accurately captures the characteristics of the corresponding LLM $k$.
Therefore, it is imperative to ensure that $a_k$\mycmt{(resp. $\rho_{a}$)} accurately captures the connection between the potential-to-see questions and the expertise of LLM $k$\mycmt{(resp. $a$)}.
In this section, we introduce \emph{Category-Calibrated Fine-Tuning (CCFT)}, a generic method for learning $a$ via contrastive fine-tuning combined with categorical weighting.


% The failure cases in Section~\ref{sec:failure_cases} show that a careful design of the model embedding $a$ is needed.
% In this section, we propose Category-Calibrated Fine-Tuning (CCFT), a generic method to train $a$ via contrastive fine-tuning and categorical weighting.
% Note that by design, $\phi(x_t, a)$ combines the information from the user side, $x_t$, and the information from the LLM side, $a$.  
% Therefore, it is imperative to make sure that $a_k$ captures the characteristics of LLM $k$.
Suppose the questions can be divided into $M$ categories\footnote{A category can refer to a topic, a benchmark, or query type, depending on the dataset.}, such as fashion, opinion, history, biology, finance, and so on.
The 3D t-SNE plot of the failure examples in Figure~\ref{fig:tsne-3d} shows that the text model tends to cluster questions from the same category.
It provides contrastive fine-tuning a good starting point.
Thus, we fine-tune the text model using a small offline question set that is disjoint from the online testing set.
Then, for each category $m$, we compute the category embedding $\xi_m$ by averaging the embeddings of offline questions belonging to that category, as generated by the fine-tuned text model. 
Note that the category embedding $\xi_m$ is not the model embedding $\rho_k$, for which an additional step is required, as described next.

To capture the unique characteristics of each LLM, we assume that every LLM is associated with a distinct Kiviat diagram, representing its areas of expertise.
Under this assumption, a natural approach is to compute a weighted combination of the category embeddings, where the weights are derived from the LLM’s scores on its Kiviat diagram. We refer to this mechanism as ``categorical weighting''.
In particular, we propose the following four weighting methods.
Denote $M$ category embeddings $(\xi_1, \xi_2, \ldots, \xi_M) := \xi$.
For each LLM $a_k$, let $(s_{k,1}, s_{k,2}, \ldots, s_{k,M})^{\top} := s_k$ be the score vector over the categories.
The first weighting method, coined ``\texttt{perf}'', defines the model embedding of $a_k$ as
\eqary{
    \rho_k = \xi \operatorname{softmax}(s_k) , 
    \num\label{eq:def_perf}
}
where $s_{k,m}$ is the model performance on category $m$.
If the score $s_{k,m}$ is a function of model performance and model cost, we coin the resulting $\rho_k$ ``\texttt{perf\_cost}''.
Note that \texttt{perf} and \texttt{perf\_cost} take all score values into account.
In reality, a common scenario involves a few strong models that specialize in different categories, alongside several weaker models that perform comparably within specific domains.
In such a case, we could weight an LLM only on categories it is good at, and leave the other categories handled by other LLMs.
Formalizing this idea, we propose ``\texttt{excel\_perf\_cost}'' as
\eqary{
    \rho_k = \xi \operatorname{softmax}\left(\operatorname{top}^{(\tau)}(s_k) \right),
    \num\label{eq:def_excel_perf_cost}
}
and ``\texttt{excel\_mask}'' as
\eqary{
    \rho_k = \xi \frac{\operatorname{mask}^{(\tau)}(s_k)}{\tau}.
    \num\label{eq:def_excel_mask}
}
Let $\tau \in [K]$, and let $s_{(\tau),m}$ denote the $\tau$-th largest value in $\{ s_{1,m}, s_{2,m}, \ldots, s_{K,m} \}$\footnote{Sorting $\{ s_{1,m}, s_{2,m}, \ldots, s_{K,m} \}$ results in $s_{(1),m} \geq s_{(2),m} \geq \ldots \geq s_{(K),m}$, and $s_{(\tau),m}$ will be located at the $\tau$-th position.}.
Function $\operatorname{top}^{(\tau)}(s_k)$ produces a real-valued vector with $m$-th entry $\operatorname{top}^{(\tau)}(s_k)_{m} = s_{k,m} \mathbf{1}[s_{k,m} \geq s_{(\tau),m}]$.
Similarly, function $\operatorname{mask}^{(\tau)}(s_k)$ produces a binary vector with $m$-th entry $\operatorname{mask}^{(\tau)}(s_k)_{m} = \mathbf{1}[s_{k,m} \geq s_{(\tau),m}]$.
% Let $\tau \in [M]$, and let $s_{k,(\tau)}$ denote the $\tau$-th largest value in $s_k$. 
% Function $\operatorname{top}^{(\tau)}(s_k)$ produces a real-valued vector with $m$-th entry
% \eqary{
%     \operatorname{top}^{(\tau)}(s_k)_{m} = s_{k,m} \mathbf{1}[s_{k,m} \geq s_{(\tau),m}] = 
%     \begin{cases}
%         s_{k,m} & \text{if } s_{k,m} \geq s_{(\tau),m},\\
%         0 & \text{otherwise.}
%     \end{cases}
% }
% Function $\operatorname{mask}^{(\tau)}(s_k)$ produces a binary vector with $m$-th entry
% \eqary{
%     \operatorname{mask}^{(\tau)}(s_k)_{m} = \mathbf{1}[s_{k,m} \geq s_{(\tau),m}] = 
%     \begin{cases}
%         1 & \text{if } s_{k,m} \geq s_{(\tau),m},\\
%         0 & \text{otherwise.}
%     \end{cases}
% }

Now, we have three ways of computing an LLM embedding.
The main idea behind these mechanisms is that the scores reflect the expertise of an LLM over the categories, the category embeddings abstract the potential-to-see questions, and the definitions $\rho_k$ show how we model the connection of these two key factors.


\subsubsection{Categorical Weighting without Scores}

Note that the weighting mechanisms (\ref{eq:def_perf}), (\ref{eq:def_excel_perf_cost}), and (\ref{eq:def_excel_mask}) require score information, which might not always be the case.
Next, we show that we can still perform a way of categorical weighting under a mild condition.

Suppose the label of a question records its best matching LLM.
Thus, we use $f_{km}$ to denote the proportion\footnote{\bcmt{A future potential: A new project of LLM + label proportion?}} of label $k$ in category $m$.
We next assume the offline data is generated as follows:
From each category $m$, a set of questions $\mathcal{Q}_m$ of size $n$ is sampled.
The offline data is $\{ \mathcal{G}_k \}_{k=1}^{K}$, formed by regrouping $\{ \mathcal{Q}_m \}_{m=1}^{M}$ according to the labels.
Given $\mathcal{G}_k$, we propose to compute the model embedding of $a_k$ by averaging over the question embeddings: Let $h$ be an embedding function and $q \in \mathcal{G}_k$ be a question. For each LLM $a_k$,
\eqary{
    % \rho_k = \frac{\sum_{q \in \mathcal{G}_k} h(q)}{|\mathcal{G}_k|}.
    \rho_k = \sum_{q \in \mathcal{G}_k} h(q) / |\mathcal{G}_k|.
    \num\label{eq:def_mix_inst}
}
The following proposition justifies the proposed mechanism.
\begin{proposition}
    % Let $h$ be an embedding function and 
    Let $\mathcal{Q}_m$ be the set of questions of size $n$ uniformly sampled from category $m$.
    Denote the proportion of label $k$ in category $m$ as $f_{km}$\footnote{ W.l.o.g., we assume $f_{km} n$ is an integer for all $k, m$.}.
    Let $Q_m$ be a random variable of questions of category $m$ sampled uniformly at random and $\mathbb{E}[h(Q_m)]$ be the expected question embedding.
    Suppose $\{ \mathcal{G}_k \}_{k=1}^{K} \}$ are given, where $\mathcal{G}_k$ gathers all questions labeled $k$ in $\{ \mathcal{Q}_m \}_{m=1}^{M}$.
    For each $k \in [K]$, the average embedding calculated from $\mathcal{G}_k$ is an unbiased estimate for
    \eqary{
        \sum_{m=1}^{M} \frac{f_{km}}{\sum_{j=1}^{M} f_{kj}} \mathbb{E}[h(Q_m)].
    }
\end{proposition}
\begin{proof}
    Let $k$ be fixed.
    % Let $q$ be a question.
    Note that the size of $\mathcal{G}_k$ is $\sum_{j=1}^{M} f_{kj} n$.
    Then,
    \eqary{
        \frac{\sum_{q \in \mathcal{G}_k} h(q)}{|\mathcal{G}_k|}
        =\ &
        \frac{\sum_{m=1}^{M} \sum_{q \in \mathcal{Q}_m} h(q)}{\sum_{j=1}^{m} f_{kj} n} 
        =\ 
        \sum_{m=1}^{M} \frac{f_{km} n}{\sum_{j=1}^{M} f_{kj} n} \frac{\sum_{q \in \mathcal{Q}_m} h(q)}{f_{km} n}.
    }
    Hence, we have the proposition by noting that $\frac{\sum_{q \in \mathcal{Q}_m} h(q)}{f_{km} n}$ is an unbiased estimation for $\mathbb{E}[h(Q_m)]$.
\end{proof}

The proposition shows that, even if there is no score information available, averaging over question embeddings still offers a way of categorical weighting in terms of label proportions: the weighting coefficients are $ \frac{f_{km}}{\sum_{j=1}^{M} f_{kj}}, m=1, \ldots, M$.
Note that a constraint is the constant $n$ over categories.
The constraint can be relaxed if we know the number of samples from each category.
Furthermore, when a pool of pairwise comparison results is gathered, one can build a rank over LLMs to determine the best matching model. 
Therefore, the $\{ \mathcal{G}_k \}$ setting and the proposed model embedding mechanism in this section fit naturally into many industrial applications.












\section{Experiments}
\label{sec:experiments}
\mycmt{(FGTS.CDB and its SGLD module)}
We implemented FGTS.CDB shown in Algorithm~\ref{alg:fgts-cdb}. 
Sampling from the posterior $p^j(\theta \mid S_{t-1})$ in Step 5 is implemented by the Stochastic Gradient Langevin Dynamics (SGLD) algorithm \citep{welling2011GDLD}.

\mycmt{(Text embedding models)}
Four text embedding models are chosen to generate embeddings for queries.
They are: OpenAI's \texttt{text-embedding-3-large} \citep{openai-text-embedding-3-large}, \texttt{all-MiniLM-L6-v2} \citep{sentence-transformers-all-MiniLM-L6-v2}, \texttt{all-mpnet-base-v2} \citep{sentence-transformers-all-mpnet-base-v2}, and \texttt{intfloat/e5-base} \citep{wang2022e5}.
In this paper, we refer to the models as \texttt{OpenAItext}, \texttt{MiniLM}, \texttt{mpnet}, and \texttt{e5b}, respectively.
\texttt{OpenAItext} serves as a strong and general-purpose embedding model.
We compare its embeddings with those generated by the fine-tuned \texttt{MiniLM}, \texttt{mpnet}, and \texttt{e5b} models to examine their impact on the feature function $\phi(x, a)$ derived from a text model.

\mycmt{(Contrastive fine-tuning)}
The fine-tuning for an open-sourced text embedding model is implemented by contrastive learning \citep{Khosla20SCL, Nils2019sentenceBERT}. 
We first build similar/dissimilar query pairs according to their source category or benchmark.
Then, the cosine-similarity loss is used to fine-tune the model.
For instance, \texttt{eb5\_E4} means that \texttt{eb5} is fine-tuned for four epochs, and \texttt{mpnet\_E2} represents \texttt{mpnet} fine-tuned for two epochs. 

\mycmt{(Prompting OpenAI's \texttt{text-embedding-3-large})}

\subsection{RouterBench}
\label{sec:exp_routerb}
RouterBench \citep{hu2024routerbench} is a comprehensive benchmark designed for evaluating LLM routing methods. 
It provides over 405k precomputed inference outputs from eleven diverse LLMs across seven tasks (MMLU, MT-Bench, MBPP, HellaSwag, Winogrande, GSM8K, ARC). 
The dataset includes detailed performance and cost metadata, enabling systematic analysis of routing strategies.
The metadata, organized into a table in \cite{hu2024routerbench} is included as Table~\ref{table:Table_1_routerb} in Appendix~\ref{sec:more_categorical_weighting}.

Next, we describe how to use the metadata and the queries in each benchmark to construct the model embedding $\rho_k$ for LLM $a_k$.
The learning process is divided into two phases: an offline fine-tuning phase, during which the model embeddings are learned, and an online testing phase, where a realization of FGTS.CDB is evaluated through a sequence of queries. 
To apply the proposed method, we need to compute $s_k$ and $\xi$.
Each benchmark $m$ is treated as a distinct category. 
To compute the corresponding category embedding $\xi_m$, we apply a text embedding model to five queries sampled from benchmark $m$, and then take the average of their embeddings.
\mycmt{(compare; distinctive) We only need 35 queries vs. MixLLM needs 30\% of the data.}
These sampled queries are excluded from the online learning phase to prevent data leakage.
Suppose \texttt{e5b\_E4} is applied to generate the embedding, then we obtain $\xi^{(\texttt{e5b\_E4})} = \left( \xi_{\textrm{MMLU}}^{(\texttt{e5b\_E4})}, \xi_{\textrm{MT-Bench}}^{(\texttt{e5b\_E4})}, \ldots, \xi_{\textrm{ARC}}^{(\texttt{e5b\_E4})} \right)$.

\begin{table*}[htbp]
\centering
\caption{Scores of \texttt{Perf\_cost}, \texttt{Excel\_perf\_cost}, and \texttt{Excel\_mask}}
\label{table:weighting}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccccccccccccccccccccccc}
\toprule
\textbf{LLM} & 
\multicolumn{3}{c}{\textbf{MMLU}} & 
\multicolumn{3}{c}{\textbf{MT-Bench}} & 
\multicolumn{3}{c}{\textbf{MBPP}} & 
\multicolumn{3}{c}{\textbf{HellaSwag}} & 
\multicolumn{3}{c}{\textbf{Winogrande}} & 
\multicolumn{3}{c}{\textbf{GSM8k}} & 
\multicolumn{3}{c}{\textbf{ARC}} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}
\cmidrule(lr){11-13}
\cmidrule(lr){14-16}
\cmidrule(lr){17-19}
\cmidrule(lr){20-22}
& (i) & (ii) & (iii) 
& (i) & (ii) & (iii) 
& (i) & (ii) & (iii) 
& (i) & (ii) & (iii) 
& (i) & (ii) & (iii) 
& (i) & (ii) & (iii) 
& (i) & (ii) & (iii) \\
% & (\ref{eq:def_perf}) & (\ref{eq:def_excel_perf_cost}) & (\ref{eq:def_excel_mask}) 
% & (\ref{eq:def_perf}) & (\ref{eq:def_excel_perf_cost}) & (\ref{eq:def_excel_mask}) 
% & (\ref{eq:def_perf}) & (\ref{eq:def_excel_perf_cost}) & (\ref{eq:def_excel_mask}) 
% & (\ref{eq:def_perf}) & (\ref{eq:def_excel_perf_cost}) & (\ref{eq:def_excel_mask}) 
% & (\ref{eq:def_perf}) & (\ref{eq:def_excel_perf_cost}) & (\ref{eq:def_excel_mask}) 
% & (\ref{eq:def_perf}) & (\ref{eq:def_excel_perf_cost}) & (\ref{eq:def_excel_mask}) 
% & (\ref{eq:def_perf}) & (\ref{eq:def_excel_perf_cost}) & (\ref{eq:def_excel_mask}) \\
\midrule
WizardLM 13B     & 0.562 & 0 & 0 & 0.796 & 0 & 0 & 0.363 & 0 & 0 & 0.600 & 0 & 0 & 0.510 & 0 & 0 & 0.492 & 0 & 0 & 0.657 & 0 & 0 \\
Mistral 7B       & 0.558 & 0 & 0 & 0.779 & 0 & 0 & 0.349 & 0 & 0 & 0.517 & 0 & 0 & 0.561 & 0 & 0 & 0.399 & 0 & 0 & 0.640 & 0 & 0 \\
Mixtral 8x7B     & 0.721 & 0.721 & 1 & 0.920 & 0.920 & 1 & 0.572 & 0.572 & 1 & 0.634 & 0 & 0 & 0.673 & 0.673 & 1 & 0.485 & 0 & 0 & 0.837 & 0.837 & 1 \\
Code Llama 34B   & 0.553 & 0 & 0 & 0.795 & 0 & 0 & 0.464 & 0 & 0 & 0.431 & 0 & 0 & 0.612 & 0 & 0 & 0.424 & 0 & 0 & 0.635 & 0 & 0 \\
Yi 34B           & 0.727 & 0.727 & 1 & 0.937 & 0.937 & 1 & 0.331 & 0 & 0 & 0.834 & 0.834 & 1 & 0.743 & 0.743 & 1 & 0.509 & 0.509 & 1 & 0.873 & 0.873 & 1 \\
GPT-3.5          & 0.700 & 0.700 & 1 & 0.907 & 0.907 & 1 & 0.649 & 0.649 & 1 & 0.695 & 0.695 & 1 & 0.623 & 0.623 & 1 & 0.543 & 0.543 & 1 & 0.844 & 0.844 & 1 \\
Claude Instant V1& 0.368 & 0 & 0 & 0.862 & 0 & 0 & 0.547 & 0 & 0 & 0.704 & 0.704 & 1 & 0.507 & 0 & 0 & 0.561 & 0.561 & 1 & 0.812 & 0 & 0 \\
Llama 70B        & 0.629 & 0 & 0 & 0.853 & 0 & 0 & 0.300 & 0 & 0 & 0.627 & 0 & 0 & 0.498 & 0 & 0 & 0.486 & 0 & 0 & 0.784 & 0 & 0 \\
Claude V1        & 0.312 & 0 & 0 & 0.920 & 0.920 & 1 & 0.497 & 0 & 0 & -0.131 & 0 & 0 & 0.516 & 0 & 0 & 0.099 & 0 & 0 & 0.798 & 0 & 0 \\
Claude V2        & 0.456 & 0 & 0 & 0.840 & 0 & 0 & 0.567 & 0.567 & 1 & -0.554 & 0 & 0 & 0.392 & 0 & 0 & -0.011 & 0 & 0 & 0.454 & 0 & 0 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

We then use the metadata in Table~\ref{table:Table_1_routerb} and the induced Table~\ref{table:weighting} to calculate the scores $s_k$.
The most straightforward way is to take only the performance columns in Table~\ref{table:Table_1_routerb}, which we call \texttt{Perf}.
For instance, taking the performance values in the fifth row of Table~\ref{table:Table_1_routerb}, we obtain $s_{\textrm{Yi 34B}}^{(\texttt{Perf})} = (0.743, 0.938, \ldots, 0.882)$.
We also implement three other scoring ways, \texttt{Perf\_cost}, \texttt{Excel\_perf\_cost}, and \texttt{Excel\_mask}. 
Using the Perf and the Cost columns in Table~\ref{table:Table_1_routerb}, scores of \texttt{Perf\_cost} is calculated by $\textrm{Perf} - \lambda \textrm{Cost}$ with $\lambda = 0.05$ being a balance parameter.
The resulting values are listed in the columns of Table~\ref{table:weighting} indexed by (i).
With \texttt{Perf\_cost} in hand, \texttt{Excel\_perf\_cost} keeps the original \texttt{Perf\_cost} score if it is ranked as the top-$\tau$ in the column and assigns $0$ otherwise. 
Here we choose $\tau=3$.
The \texttt{Excel\_perf\_cost} scores are listed under index (ii).
\texttt{Excel\_mask} further masks the nonzero values of \texttt{Excel\_perf\_cost} as $1$ and lists them under (iii) in Table~\ref{table:weighting}. 
Finally, we feed the scores $s_k$ and the model embeddings $\xi$ to (\ref{eq:def_perf}), (\ref{eq:def_excel_perf_cost}), and (\ref{eq:def_excel_mask}) to obtain the model embedding $\rho_k$.
Specifically, \texttt{Perf} and \texttt{Perf\_cost} are fed to (\ref{eq:def_perf}), \texttt{Excel\_perf\_cost} to (\ref{eq:def_excel_perf_cost}), and \texttt{Excel\_mask} to (\ref{eq:def_excel_mask}).
Using the above symbols, we can denote, for instance, the model embedding of Yi 34B calculated via text embedding model \texttt{e5b\_E4}, scoring method \texttt{Perf\_cost}, and weighting equation (\ref{eq:def_perf}) as 
$
\rho_{\textrm{Yi 34B}}^{(\texttt{e5b\_E4\_}\texttt{Perf\_cost})} = \xi^{(\texttt{e5b\_E4})} \operatorname{softmax}\left(s_{\textrm{Yi 34B}}^{(\texttt{Perf\_cost})}\right)\footnote{Note that \texttt{e5b}, \texttt{mpnet}, and \texttt{MiniLM} are text models that generate embeddings. They need to be distinguished from the LLMs, listed in the leftmost column of Table~\ref{table:weighting}, which are candidates selected to generate responses in online learning.}.
$ 
In addition, we append all $14$ metadata (Perf and Cost over seven benchmarks) of an LLM at the end of its embedding.
Let $\rho_{x}$ be the embedding of query $x$, the feature function $\phi(x, a_k)$ is computed as the normalized $\rho_{x} * \rho_{k}$. 
To compare the effectiveness of fine-tuning, we use a suffix to indicate whether a fine-tuned model or an original model generates an embedding. 
For instance, the string ``\texttt{e5b\_E4\_Excel\_perf\_cost\_exp}'' means ``belonging to the experimental group, the embedding is generated by \texttt{e5b} fine-tuned with four epochs with the \texttt{Excel\_perf\_cost} weighting mechanism'', and ``\texttt{e5b\_E4\_Excel\_perf\_cost\_ctrl}'' means ``belonging to the control group, the embedding is generated by the original \texttt{e5b} with the \texttt{Excel\_perf\_cost} weighting mechanism.

We run \texttt{OpenAItext} with one, three, and five queries, each for five runs, and average the cumulative regrets to plot three curves\footnote{Unless mentioned, each regret curve reported is the average of 5 runs.} in Figure~\ref{fig:rtb-main-a}.
\mycmt{Is it 1, 3, and 5 or one, three, and five?}
For open-sourced embdeeing models, we fine-tune to obtain \texttt{e5b\_E2}, \texttt{e5b\_E4}, \texttt{mpnet\_E2}, \texttt{mpnet\_E4}, \texttt{MiniLM\_E2}, and \texttt{MiniLM\_E4}.
For each embedding model, four weighting mechanisms (\texttt{Perf}, \texttt{Perf\_cost}, \texttt{Excel\_perf\_cost}, \texttt{Excel\_mask}) are implemented.
The corresponding control group also undergoes the online testing phase.
There are a total of 8 curves for one embedding model.
The best performed \texttt{e5b\_E4} is shown in Figure~\ref{fig:rtb-main-b}. 
Results for the other models can be found in Figure~\ref{fig:grid-rtb-models-all} from Appendix~\ref{sec:more_routerb_results}.

We obtain the following observations from the regret curves.
In Figure~\ref{fig:rtb-main-a}, the number of queries in the prompt does not affect \texttt{OpenAItext} too much.
Thus, we choose the best version, \texttt{openai\_4}, to compare with the results generated by our proposed CCFT in Figure~\ref{fig:rtb-main-b}.
First, the experimental group outperforms the control group, showing the advantage of fine-tuning.
Second, \texttt{e5b\_E4\_Excel\_perf\_cost\_exp} and \texttt{e5b\_E4\_Excel\_mask\_exp} outperform \texttt{openai\_4}, showing that even an open-sourced model, with a careful design, can generate better embeddings than a strong general-purpose model. 
Third, when examining all plots in Figure~\ref{fig:grid-rtb-models-all-b} -- \ref{fig:grid-rtb-models-all-f}, the previous two observations hold for all other embedding models, showing convincing evidence for the effectiveness of CCFT we proposed.
Fourth, by comparing \texttt{e5b\_E4\_Excel\_perf\_cost\_exp} with \texttt{e5b\_E4\_Perf\_cost\_exp}, we observe that weighting via \texttt{Excel\_perf\_cost} yields better performance than weighting via \texttt{Excel\_mask}.
\mycmt{We compare with $a^*_{t}$, not just $a^*$.}
This suggests that, instead of weighting over all categories, it is more effective to weight only the categories in which the LLM demonstrates expertise.
In addition to achieving lower accumulated regret, both \texttt{Excel\_perf\_cost} and \texttt{Excel\_mask} incorporate a performance-cost trade-off, enhancing their practical applicability and flexibility through the tunable parameter $\lambda$.
\mycmt{Compare our TS vs MixLLM's UCB approach?}

% --- 1x2 layout ---
\begin{figure}[t]
  \centering
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{routerb_seed2_m42_set4_figure_0.png}
    \caption{\texttt{OpenAItext} results}
    \label{fig:rtb-main-a}
  \end{subfigure}\hfill
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{routerb_seed1_m42_set1_figure_0.png}
    \caption{Fine-tuned results}
    \label{fig:rtb-main-b}
  \end{subfigure}

  \caption{RouterBench: Cumulative regret curves (lower is better).}
  \label{fig:rtb-main}
\end{figure}
% --- 1x2 layout ---








\subsubsection{Generalization to an Unseen Benchmark}

Although an online learning setting evaluates an algorithm’s adaptivity by providing sequentially and randomly shuffled inputs, the algorithm may still access metadata from all benchmarks during the offline stage.
To more rigorously assess adaptivity to an unseen benchmark, we modify the data-generation pipeline to ensure that one benchmark remains completely hidden from the algorithm throughout both the offline and online phases.
The queries and metadata of MT-Bench are removed, as its dataset is not large enough to induce a distribution shift scenario in the coming experiment.
For the remaining six benchmarks, the metadata for ARC is removed from Table~\ref{table:Table_1_routerb}, ensuring that the algorithm is oblivious to it from the outset.
An online learning sequence is composed of two sections.
First, we sample 60 queries from each benchmark, excluding ARC (i.e., five benchmarks in total), resulting in 300 queries. 
These are randomly shuffled to form the first section of the sequence.
Next, for the second section, we sample 120 queries from ARC and an additional 300 non-overlapping queries from the other five benchmarks, following the same procedure as in the first section. These 420 (i.e., $120 + 300$) queries are then shuffled to form the second section of the learning sequence.
This setup introduces a shift in the query distribution during the second section of online learning, as queries from a previously unseen benchmark are added to evaluate the robust generalization capability of the proposed method.
Due to the modification in how metadata is accessed, we introduce an additional suffix, \texttt{ideal}, which allows the model to access ARC's metadata.
Although the \texttt{ideal} case is not realistic in practice, comparing results from configurations ending with \texttt{ideal} and those ending with \texttt{exp} enables us to assess the adaptivity strength of our method.
For the rest of the experimental setting, we follow the same fine-tuning protocol in the last section to generate embeddings.
Based on the observations from Figures~\ref{fig:rtb-main-b} and~\ref{fig:grid-rtb-models-all}, we implement the \texttt{Excel\_perf\_cost} and \texttt{Excel\_mask} weighting schemes due to their consistently strong performance.

The results of \texttt{OpenAItext} and \texttt{e5b} are shown in Figure~\ref{fig:rbst-main}.
Results for \texttt{mpnet} and \texttt{MiniLM} can be found in Figure~\ref{fig:rtb-rbst-all} from Appendix~\ref{sec:more_routerb_results}.
We choose \texttt{openai\_0} to compare with the results generated by \texttt{e5b\_E4} according to Figure~\ref{fig:rbst-main-a}.
First, obviously, the fine-tuning group outperforms the control group.
Second, \texttt{e5b\_E4\_Excel\_perf\_cost\_exp} and \texttt{e5b\_E4\_Excel\_mask\_exp}, the fine-tuning results via our CCFT method outperform that of \texttt{openai\_0}.
The case in the second observation holds for Figure~\ref{fig:rtb-rbst-all-a} through Figure~\ref{fig:rtb-rbst-all-e}, justifying the effectiveness of the proposed method.
\mycmt{However, due to the unseen benchmark, the curve gaps between \texttt{openai\_0} become closer (REALLY?) to that in Figure~\ref{fig:rtb-main-b}. I need to plot a figure to compare. Maybe openai\_0 suffers more in unseen benchmark.} 
Third, interestingly, we find that it is not always the case that an \texttt{ideal} curve outperforms the corresponding \texttt{exp} curve.
One can find this by comparing pair (\texttt{e5b\_E4\_Excel\_perf\_cost\_exp}, \texttt{e5b\_E4\_Excel\_perf\_cost\_ideal}) with pair (\texttt{e5b\_E4\_Excel\_mask\_exp}, \texttt{e5b\_E4\_Excel\_mask\_ideal}).
The situation also can be found in Figure~\ref{fig:rtb-rbst-all}.
\mycmt{In particular, in Figure~\ref{fig:rtb-rbst-all-d} and \ref{fig:rtb-rbst-all-e}.}
This phenomenon suggests weighting less may be better than weighting more, and it may be related to the last observation we have in the original RouterBench experiments that weighting over all benchmark embeddings is not a good idea.
Maybe the metadata alone is not enough for us to make a weighting judgment; we might need to look into other aspects of the benchmarks in future work.



\begin{figure}[t]
  \centering
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{routerb_rbst2_m42_set4_figure_0.png}
    \caption{OpenAI variants}
    \label{fig:rbst-main-a}
  \end{subfigure}\hfill
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{routerb_rbst1_m42_set1_figure_0.png}
    \caption{E5b variants}
    \label{fig:rbst-main-b}
  \end{subfigure}

  \caption{Robust generalization: Cumulative regret curves (lower is better).}
  \label{fig:rbst-main}
\end{figure}








\subsection{MixInstruct}
\label{sec:exp_mixInst}
MixInstruct \citep{jiang2023mixinst_blender} is a 110K-example instruction-following benchmark built to evaluate LLM routing methods. 
It mixes data from four sources (Alpaca-GPT4, Dolly-15K, GPT4All-LAION, ShareGPT) with a 100k/5k/5k train/dev/test split. 
The authors run eleven popular open-source LLMs on the full set, then derive oracle pairwise preferences by prompting ChatGPT to compare every candidate pair per example.

\begin{table}[h!]
\caption{Models Ranked First by Percentage of Examples}
\label{table:mix-inst-top-percentage}
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lccccccccccc}
\toprule
\textbf{Model} & Vicuna & MOSS & Open Assistant & Alpaca & Baize & ChatGLM & MPT & Koala & Dolly V2 & StableLM & FLAN-T5 \\
\midrule
\textbf{Percentage (\%)} & 21.22 & 12.91 & 12.61 & 11.61 & 11.61 & 8.51 & 7.61 & 6.71 & 4.50 & 1.90 & 0.80 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
% \mycmt{MixInstruct table is generated by \url{https://chatgpt.com/c/68cc1655-c370-8322-8021-c70b7cb8ea78}.}

Table~\ref{table:mix-inst-top-percentage}, adapted from Figure 1 of \cite{jiang2023mixinst_blender}, underscores the importance of LLM routing: selecting the best-matching LLM for each query is crucial, as any fixed-LLM strategy will yield no more than 22\% accuracy.
A distinctive characteristic of the MixInstruct dataset is the absence of an explicit category label, rendering the proposed methods in (\ref{eq:def_perf}), (\ref{eq:def_excel_perf_cost}), and (\ref{eq:def_excel_mask}) infeasible.
Since this challenge can naturally arise in practical settings, we use MixInstruct to evaluate our alternative formulation presented in (\ref{eq:def_mix_inst}), thereby validating its applicability under realistic constraints.
Moreover, the pairwise comparison labels in MixInstruct make it closely resemble datasets commonly encountered in industrial applications.

To make the regret defined in (\ref{eq:regret}) computable, we reconstruct the utility function $r^{*}(x, a)$.
Pairwise comparisons between LLM candidates are translated into scores by adding a win value of 1, a tie 0.5, and a loss 0.
During the translation process, a Condorcet winner may emerge \citep{black1958,wiki_condorcet_winner}. 
To ensure it receives the highest score, we assign the Condorcet winner a top score with an additional bonus.
During the data analysis stage, we found the existence of ambiguous queries. 
We apply the OpenAI API to assign an ambiguity score to each query and remove the most ambiguous 8\% and 15\% of queries.
The ambiguity removal process introduces additional sub-strings \texttt{\_8} and \texttt{\_15} in the naming of regret curves. 
Using (\ref{eq:def_mix_inst}), the rest of the experiment setup follows the procedure described in Section~\ref{sec:exp_routerb}.
We obtain Figure~\ref{fig:mixinst-main} and deferred Figure~\ref{fig:mixinst-15} to Appendix~\ref{sec:more_mixinst} due to space limit.

\begin{figure}[h]
  \centering
  % Left plot
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{mixinst_seed_m1_set1_figure_0.png}
    \caption{Implementations of (\ref{eq:def_mix_inst}) versus \texttt{openai} variants}
    \label{fig:mixinst-main-8}
  \end{subfigure}\hfill
  % Right plot
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{mixinst_seed_m1_set2_figure_0.png}
    \caption{Comparing ambiguity removal: 8\% versus 15\%}
    \label{fig:mixinst-main-compare}
  \end{subfigure}

  \caption{MixInstruct: Cumulative regret curves (lower is better).}
  \label{fig:mixinst-main}
\end{figure}

In Figure~\ref{fig:mixinst-main-8}, we again observe that implementations of the proposed (\ref{eq:def_mix_inst}) outperform \texttt{openai} variants, demonstrating that our approach remains effective even when the dataset lacks metadata information.
When comparing results under different degrees of ambiguity removal, we observe a consistent pattern in Figure~\ref{fig:mixinst-main-compare} across \texttt{e5b\_E4}, \texttt{mpnet\_E4}, and \texttt{openai\_4}: removing the top 15\% of ambiguous queries is worse than removing only the top 8\%. 
This highlights the risk of discarding learnable information when too many queries are removed.




\section{Concluding Remarks and Future Work}

(1) Integrate the preference feedback and rating scale feedback.
Our method considers dueling feedback currently. 
It can be easily modified to take rating scale feedback.
However, a challenge is to integrate both. 
It is unclear how to build an online learner that takes both forms of input.

(2) Dynamically retrain the model embedding.
The proposed model embedding is trained by a fixed offline dataset.
As time goes on, the service provider will receive new annotated information.
It would be interesting to construct a mechanism that adapts the model embedding to reflect the newly available dataset.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection*{Author Contributions}
% Optional.

% \subsubsection*{Acknowledgments}
% \mycmt{All acknowledgments, including those to funding agencies, go at the end of the paper.}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibliography{iclr2026/bibtex_llm-routing}
\bibliographystyle{iclr2026_conference}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage

\appendix


\section{MMLU Supplementary Materials}
\label{sec:more_mmlu}

\begin{figure*}[h]
  \centering
  \includegraphics[width=0.95\linewidth]{tsne_3d_side_by_side.png}
  \caption{3D t-SNE visualization of experimental (left) and control (right) groups. Each point represents an embedding projected into 3D space, with colors indicating cluster membership.}
  \label{fig:tsne-3d}
\end{figure*}
\mycmt{t-SNE and 3D t-SNE plots?}



\section{RouterBench Supplementary Materials}
\label{sec:more_routerb}


\subsection{Categorical Weighting}
\label{sec:more_categorical_weighting}

\begin{table}[htbp]
\centering
\caption{Performance and cost across benchmarks}
\label{table:Table_1_routerb}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccccccccccccc}
\toprule
\textbf{LLM} & 
\multicolumn{2}{c}{\textbf{MMLU}} & 
\multicolumn{2}{c}{\textbf{MT-Bench}} & 
\multicolumn{2}{c}{\textbf{MBPP}} & 
\multicolumn{2}{c}{\textbf{HellaSwag}} & 
\multicolumn{2}{c}{\textbf{Winogrande}} & 
\multicolumn{2}{c}{\textbf{GSM8k}} & 
\multicolumn{2}{c}{\textbf{ARC}} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
\cmidrule(lr){8-9}
\cmidrule(lr){10-11}
\cmidrule(lr){12-13}
\cmidrule(lr){14-15}
& Perf$\uparrow$ & Cost$\downarrow$ 
& Perf$\uparrow$ & Cost$\downarrow$ 
& Perf$\uparrow$ & Cost$\downarrow$ 
& Perf$\uparrow$ & Cost$\downarrow$ 
& Perf$\uparrow$ & Cost$\downarrow$ 
& Perf$\uparrow$ & Cost$\downarrow$ 
& Perf$\uparrow$ & Cost$\downarrow$ \\
\midrule
WizardLM 13B     & 0.568 & 0.122 & 0.796 & 0.006 & 0.364 & 0.011 & 0.636 & 0.727 & 0.512 & 0.040 & 0.510 & 0.354 & 0.660 & 0.068 \\
Mistral 7B       & 0.562 & 0.081 & 0.779 & 0.003 & 0.349 & 0.006 & 0.541 & 0.485 & 0.562 & 0.027 & 0.409 & 0.210 & 0.642 & 0.046 \\
Mixtral 8x7B     & 0.733 & 0.245 & 0.921 & 0.012 & 0.573 & 0.023 & 0.707 & 1.455 & 0.677 & 0.081 & 0.515 & 0.594 & 0.844 & 0.137 \\
Code Llama 34B   & 0.569 & 0.317 & 0.796 & 0.015 & 0.465 & 0.021 & 0.525 & 1.882 & 0.617 & 0.104 & 0.462 & 0.752 & 0.644 & 0.177 \\
Yi 34B           & 0.743 & 0.326 & 0.938 & 0.018 & 0.333 & 0.031 & 0.931 & 1.938 & 0.748 & 0.107 & 0.552 & 0.867 & 0.882 & 0.182 \\
GPT-3.5          & 0.720 & 0.408 & 0.908 & 0.026 & 0.651 & 0.044 & 0.816 & 2.426 & 0.630 & 0.134 & 0.601 & 1.170 & 0.855 & 0.228 \\
Claude Instant V1& 0.384 & 0.327 & 0.863 & 0.030 & 0.550 & 0.064 & 0.801 & 1.943 & 0.512 & 0.108 & 0.626 & 1.300 & 0.821 & 0.183 \\
Llama 70B        & 0.647 & 0.367 & 0.854 & 0.022 & 0.302 & 0.039 & 0.736 & 2.183 & 0.504 & 0.121 & 0.529 & 0.870 & 0.794 & 0.205 \\
Claude V1        & 0.475 & 3.269 & 0.938 & 0.361 & 0.527 & 0.607 & 0.841 & 19.43 & 0.570 & 1.077 & 0.653 & 11.09 & 0.889 & 1.829 \\
Claude V2        & 0.619 & 3.270 & 0.854 & 0.277 & 0.605 & 0.770 & 0.421 & 19.50 & 0.446 & 1.081 & 0.664 & 13.49 & 0.546 & 1.833 \\
GPT-4            & 0.828 & 4.086 & 0.971 & 0.721 & 0.682 & 1.235 & 0.923 & 24.29 & 0.858 & 1.346 & 0.654 & 19.08 & 0.921 & 2.286 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

Tables \ref{table:Table_1_routerb} and \ref{table:weighting} are from \url{https://chatgpt.com/c/68cb776a-3fbc-8329-b5a1-3cf59d40b1f5}


% \begin{table}[h!]
% \label{table:hypothetic_method}
% \centering
% \caption{LLM Scores Across Categories}
% \begin{tabular}{lccccccc}
% \toprule
%  & Category 1 & Category 2 & Category 3 & Category 4 & Category 5 & Category 6 & Category 7 \\
%   & $\xi_1$ & $\xi_2$ & $\xi_3$ & $\xi_4$ & $\xi_5$ & $\xi_6$ & $\xi_7$ \\
% \midrule
% LLM $a_1$ & 0.368 & 0.862 & 0.547 & \textbf{0.704} & 0.507 & \textbf{0.561} & 0.812 \\
% LLM $a_2$ & 0.629 & 0.853 & 0.300 & 0.627 & 0.498 & 0.486 & 0.784 \\
% LLM $a_3$ & \textbf{0.721} & \textbf{0.920} & \textbf{0.572} & 0.634 & \textbf{0.673} & 0.485 & \textbf{0.837} \\
% LLM $a_4$ & \textbf{0.727} & \textbf{0.937} & 0.331 & \textbf{0.834} & \textbf{0.743} & \textbf{0.509} & \textbf{0.873} \\
% LLM $a_5$ & 0.456 & 0.840 & \textbf{0.567} & -0.554 & 0.392 & -0.011 & 0.454 \\
% \bottomrule
% \end{tabular}
% \end{table}

% Using the hypothetical table above, we present 
% \bcmt{(maybe move to appendix or delete).}





\subsection{Additional Results}
\label{sec:more_routerb_results}

Figure~\ref{fig:grid-rtb-models-all} lists the cumulative regret curves for \texttt{e5b\_E2}, \texttt{mpnet\_E4}, \texttt{mpnet\_E2}, \texttt{MiniLM\_E4}, and \texttt{MiniLM\_E2}.
Figure~\ref{fig:grid-rtb-models-all-a} compares all embedding models with \texttt{Excel\_perf\_cost} and \texttt{Excel\_mask} mechanisms, which are the better weighting method most of the time.

% --- 3-by-2 Figure ---
\begin{figure*}[h]
  \centering
  % Row 1
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{routerb_seed1_m42_set2_figure_0.png}
    \caption{Compare against text models.}
    \label{fig:grid-rtb-models-all-a}
  \end{subfigure}\hfill
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{routerb_seed1_m42_set1_figure_1.png}
    \caption{\texttt{e5b\_E2} results.}
    \label{fig:grid-rtb-models-all-b}
  \end{subfigure}

  \vspace{0.3em}

  % Row 2
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{routerb_seed1_m42_set1_figure_2.png}
    \caption{\texttt{mpnet\_E4} results.}
  \end{subfigure}\hfill
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{routerb_seed1_m42_set1_figure_3.png}
    \caption{\texttt{mpnet\_E2} results.}
  \end{subfigure}

  \vspace{0.3em}

  % Row 3
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{routerb_seed1_m42_set1_figure_4.png}
    \caption{\texttt{MiniLM\_E4} results.}
  \end{subfigure}\hfill
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{routerb_seed1_m42_set1_figure_5.png}
    \caption{\texttt{MiniLM\_E2} results.}
    \label{fig:grid-rtb-models-all-f}
  \end{subfigure}

  \caption{RouterBench: Cumulative regret curves (lower is better).}
  \label{fig:grid-rtb-models-all}
\end{figure*}
% --- 3-by-2 Figure ---


% % --- 2-by-3 Figure ---
% \begin{figure*}[t]
%   \centering
%   \begin{subfigure}{0.32\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{routerb_seed1_m42_set1_figure_0.png}
%     \caption{A}
%   \end{subfigure}\hfill
%   \begin{subfigure}{0.32\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{routerb_seed1_m42_set1_figure_1.png}
%     \caption{B}
%   \end{subfigure}\hfill
%   \begin{subfigure}{0.32\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{routerb_seed1_m42_set1_figure_2.png}
%     \caption{C}
%   \end{subfigure}

%   \vspace{0.3em}

%   \begin{subfigure}{0.32\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{routerb_seed1_m42_set1_figure_3.png}
%     \caption{D}
%   \end{subfigure}\hfill
%   \begin{subfigure}{0.32\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{routerb_seed1_m42_set1_figure_4.png}
%     \caption{E}
%   \end{subfigure}\hfill
%   \begin{subfigure}{0.32\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{routerb_seed1_m42_set1_figure_5.png}
%     \caption{F}
%   \end{subfigure}

%   \caption{Cumulative regret curves.}
%   \label{fig:grid-rtb-models}
% \end{figure*}
% % --- 2-by-3 Figure ---


\begin{figure*}[h]
  \centering
  % Row 1
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{routerb_rbst1_m42_set1_figure_1.png}
    \caption{A}
    \label{fig:rtb-rbst-all-a}
  \end{subfigure}\hfill
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{routerb_rbst1_m42_set1_figure_2.png}
    \caption{B}
    \label{fig:rtb-rbst-all-b}
  \end{subfigure}

  \vspace{0.3em}

  % Row 2
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{routerb_rbst1_m42_set1_figure_3.png}
    \caption{C}
    \label{fig:rtb-rbst-all-c}
  \end{subfigure}\hfill
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{routerb_rbst1_m42_set1_figure_4.png}
    \caption{D}
    \label{fig:rtb-rbst-all-d}
  \end{subfigure}

  \vspace{0.3em}

  % Row 3
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{routerb_rbst1_m42_set1_figure_5.png}
    \caption{E}
    \label{fig:rtb-rbst-all-e}
  \end{subfigure}\hfill
  % \begin{subfigure}{0.45\textwidth}
  %   \centering
  %   \includegraphics[width=\linewidth]{routerb_rbst1_m42_set1_figure_0.png}
  %   \caption{F}
  %   \label{fig:rbst3x2-f}
  % \end{subfigure}

  \caption{Robust generalization: Cumulative regret curves (lower is better).}
  \label{fig:rtb-rbst-all}
\end{figure*}

\mycmt{Figure comes from \url{https://chatgpt.com/c/68cbf7d5-e4fc-832d-a9a0-5c5c1f1c193a}.}





\section{MixInstruct Supplementary Materials}
\label{sec:more_mixinst}



\subsection{Additional Results}
\label{sec:more_mixinst_results}

\mycmt{Add Figure~\ref{fig:mixinst-fig1}.}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\linewidth]{mixinst_seed_m1_set1_figure_1.png}
  \caption{Cumulative regret curves (lower is better).}
  \label{fig:mixinst-15}
\end{figure}









==> iclr2026/97_other_stuffs.tex <==


\section{(remove from submission) More on Section~\ref{sec:failure_cases}}
\bcmt{ 
Take a common practice of enlisting a text model to generate the model embeddings and the question embeddings. 
The model embedding is generated through prompting and sampled questions.
The question embedding is generated directly.
A straight line of constant regret accumulation indicates no learning effect.
It evidence the failure of careless designed feature. 
}
\rcmt{Why OpenAI shows a straight line in mmlu but a curve in p.67, [progress\_250509]? Answer: In RouterBench and MixInstruct, additional performance values are fed into the creation process of embedding (i.e., the model\_desc part).}

Simulated results are:
\begin{itemize}
    \item fgts-llm-mmlu.py: model embedding = OpenAI + prompting + sampled questions.
    \item fgts-llm-mmlu\_250406.py: model embedding = OpenAI + sampled questions + averaging.
    \item fgts-llm-mmlu-finetune-3.py: model embedding = fine-tuned model + sample questions + averaging.
\end{itemize}






\section{(remove from submission) Materials}

(algorithm) FGTS.CDB
\url{https://chatgpt.com/c/68bd18df-022c-8332-b635-e564f6854fc8}

(terminology) rating scale feedback. pairwise preference feedback. 
\url{https://chatgpt.com/c/68bdfe8a-0e84-832a-a65f-bbaf7f550b8d}
Company: routing service
\url{https://www.helicone.ai/}
Company: langtrace
\url{https://www.langtrace.ai/}

(compare) online learning vs supervised learning
\url{https://chatgpt.com/c/68be3bcb-3ae0-8329-adf9-24775e558d46}

(naming) Choose a name for our method: Category-Calibrated Fine-Tuning (CCFT)
\url{https://chatgpt.com/c/68bf4c2c-0b20-8324-9580-9ea221ce1da2}




\section{(remove from submission) Derivation for $m = 1, 2$}
\url{https://chatgpt.com/c/68c0f6e5-4c20-8325-91d8-7ded30cd8cab}

Annotate each $q \sim C_m$ with the best matching label $L \Rightarrow f_{km}$ is the proportion of label $k$ in category $C_m$.

Suppose a question set is sampled from $C_m$, 
denoted $Q_m$, of size $n$.

Let $\{ Q_m \}_{m=1}^M$ be regrouped into $\{ G_k \}_{k=1}^K$,
where $G_k$ is the set of questions annotated with label $k$.

Then, for each $k$,

$\frac{\sum_i h(q_i)}{|G_k|},$

$|G_k| = f_{k1} n + f_{k2} n,$

$\frac{\sum_i h(q_i)}{f_{k1} n + f_{k2} n}
= \frac{f_{k1} n}{f_{k1} n + f_{k2} n} \cdot \frac{\sum_{q_i \in G_1} h(q_i)}{f_{k1} n}
+ \frac{f_{k2} n}{f_{k1} n + f_{k2} n} \cdot \frac{\sum_{q_i \in G_2} h(q_i)}{f_{k2} n}$

$= \frac{f_{k1}}{f_{k1} + f_{k2}} \cdot \frac{1}{|G_1|} \sum_{q_i \in G_1} h(q_i)
+ \frac{f_{k2}}{f_{k1} + f_{k2}} \cdot \frac{1}{|G_2|} \sum_{q_i \in G_2} h(q_i)$

which is an estimate of

$\frac{f_{k1}}{f_{k1} + f_{k2}} \mathbb{E}[h(Q_1)]
+ \frac{f_{k2}}{f_{k1} + f_{k2}} \mathbb{E}[h(Q_2)].$



==> iclr2026/98_citations_figures_tables.tex <==


% ======================================================================= %
\section{Citations, figures, tables, references}
\label{others}

\subsection{Citations within the text}

When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}





==> iclr2026/99_default_notation.tex <==

% ======================================================================= %
\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}




==> iclr2026/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

